The Explanation Game: Towards Prediction Explainability through Sparse Communication

Explainability is a topic of growing importance in NLP. In this work, we provide a unified perspective of explainability as a communication problem between an explainer and a layperson about a classifier's decision. We use this framework to compare several prior approaches for extracting explanations, including gradient methods, representation erasure, and attention mechanisms, in terms of their communication success. In addition, we reinterpret these methods at the light of classical feature selection, and we use this as inspiration to propose new embedded methods for explainability, through the use of selective, sparse attention. Experiments in text classification, natural language entailment, and machine translation, using different configurations of explainers and laypeople (including both machines and humans), reveal an advantage of attention-based explainers over gradient and erasure methods. Furthermore, human evaluation experiments show promising results with post-hoc explainers trained to optimize communication success and faithfulness.

==> BlackBoxNLP 2020 - SCE/backup_tables.tex <==
\begin{table}[!htb]
\small
\begin{center}
\begin{tabular}{l cc c cc}
\toprule
\multirow{2}{*}{\sc Method} & \multicolumn{2}{c}{\sc SNLI} & & \multicolumn{2}{c}{\sc eSNLI} \\


\cmidrule{2-3} \cmidrule{5-6}


	& $C_{\mathrm{ACC}}$ & $L_{\mathrm{ACC}}$ 	& & $C_{\mathrm{ACC}}$ & $L_{\mathrm{ACC}}$  \\

\midrule 

Bag of words    	& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
RNN softmax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
RNN sparsemax	 	& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
RNN 1.5-entmax		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\

\midrule

Uniform	 		        & 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Shuffle	 		        & 86.20   & 86.20   	& & 86.20   & 86.20   	\\

\midrule 

Erasure softmax 		& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
Erasure sparsemax		& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
Erasure 1.5-entmax	    & 86.20   & 86.20   	& & 86.20   & 86.20  	\\

\midrule

Top-k gradient    		& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
Zero-max-out softmax	& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Top-k softmax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Top-k sparsemax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Top-k 1.5-entmax		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\


\midrule

Full sparsemax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Full 1.5-entmax			& 86.20   & 86.20   	& & 86.20   & 86.20   	\\

\bottomrule
\end{tabular}
\end{center}
\caption{Results for SNLI and eSNLI.} \label{table:results_nli}
\end{table}




==> BlackBoxNLP 2020 - SCE/figs/experimental_comments.tex <==
\begin{itemize}
    \item Accuracy dos classifiers sao altas (muito proximo com os valores dos classifiers dos trabalhos relacionados - jain and wallace). 
    
    \item Falar do tamanho dos datsets nao influenciou muito
    
    \item Bag of words parece ser um strong baseline para todos os datasets. Especialmente para o AgNews
    
    \item Como esperado, usando shuffled or uniform random weights os resultados em termos de Lacc sao baixos. Exceto para o agnews, o qual usando random weights os resultados do layperson ainda sao consideravelmente altos (>90\%).
    
    \item Metodos baseados em erasure e encoded attention tem performances bem similares em termos de Lacc
    
    \item Gradient tem resultados mais baixos que erasure e attention
    
    \item Full attention (embedded) possui os melhores resultados em termos de Lacc
    
    \item Zerando a palavra com maior attention os resultados decaem comparando quando essa palavra estava inclusa, porem nao decaem tanto como quanto random, sugerindo que as palavras selecionadas via attention sao de fato relevantes. De fato, a acc desse explainer eh ate melhor que gradient explainer no IMDB e no YELP, os quais possuem sentencas muito grandes. Embora nao reportamos na tabela, resultados zerando os maiores attention scores computados via sparse attentions sao em geral um pouco melhores que usando softmax, entao a conclusao se mantem para alpha = 1.5 e 2.
    
    \item Usando attention ou erasure, os na maioria das vezes ficam melhores do que usando um bag of words completo, o que indica que a informacao relevante para a classificao esta sendo selecionada por esses explainers
    
    \item Com excecao do agnews, para os outros datasets da para perceber que sparse attentions geralmente refletem em uma maior accuracia de comunicacao. Para o agnews, descobrimos que se fizermos attention selecionando apenas as primeiras k palavras da sentenca, tanto a acc da comunicacao quanto a acc do layperson continuam muito altas (cerca de 93\%). Devido a isso, desconsideramos futuras analises para este corpus. 
    
    \item Olhando para a accuracia de comunicao podemos ver que metodos baseados em attention e erasure tambem possuem resultados melhores. 
    
    \item Novamente, olhando para os diferentes valores de alpha, percebemos que attentions mais esparsas tendem a ter uma acc de comunicacao ligeiramente maior (exceto no agnews).  
    
    \item Comparando os resultados entre encoded and embedded attention, podemos ver que em geral, a acc da comunicacao eh maior para encoded attention porem o layperson acc eh maior para embedded attention. Podemos ver tambem que para o SST e AgNews o resultado usando encoded e embedded sparsemax sao exatamente os mesmos. Isso acontece pois a distribuicao do sparsemax possui, na grande maioria das vezes, menos de $k$ nonzero probabilities, e portanto as mesmas palavras foram selecionadas pelos dois metodos. Mais adiante analisamos o impacto da esparsidade em mais detalhes.
    
    \item Em geral, esses experimentos nos mostram que, para os datasets analisados, usando palavras selecionadas via attention os resultados tanto em termos de Cacc e Lacc sao bastante apelativos, sugerindo que attention pode ser tratado como uma explicacao plausivel. Mais adiante discutimos se de fato podemos tratar as explanations desses metodos como faithfuls
\end{itemize}

==> BlackBoxNLP 2020 - SCE/related_work.tex <==
\section{Related Work}\label{sec:related_work}

%The area of explainable AI is growing very fast, with





%Recent work used the information bottleneck \citep{} minimum description principle \citep{} 
%\andre{todo: add relation to MDL principle (Voita's paper) and IB principle (Eisner's paper, see \url{https://medium.com/jasonwu0731/information-bottleneck-for-nlp-parsing-summarization-961418fbb697})}

There is a large body of work on analysis and interpretation of neural networks. 
%One area of research, not addressed in our paper, concerns understanding what different neural architectures can and cannot do, and  distilling them to models that are globally more amenable to interpretation, such as finite-state automata \citep{weiss2018practical,weiss2018extracting,schwartz2018bridging,peng2018rational}. 
Our work focuses on {\it prediction explainability}, different from transparency or model interpretability \citep{doshi2017towards,lipton2016mythos,gilpin2018explaining}.  %,riedl2019human}. 

\citet{rudin2019stop} defines explainability as a plausible reconstruction of the decision-making process, and \citet{riedl2019human} argues that it mimics what humans do when rationalizing past actions. This inspired our post-hoc explainers in \S\ref{subsec:joint_e_and_l} and their use of the faithfulness loss term. 

%The area of explainable AI is growing very fast. Several terminologies have been proposed in the last few years in order to have concise definitions of explainable AI properties \citep{lipton2016mythos,doshi2017towards}. 
%One option to obtain transparency is by developing models that are natively interpretable, such as ... \citep{rudin2019stop}, rather than attempting to explain non-transparent models. Whether this can be done without sacrificing model accuracy is currently unclear.

Recent works questioned the interpretative ability of attention mechanisms %and whether they can be regarded as a form of explanation or not
\citep{jain2019attention,serrano2019attention}. 
\citet{wiegreffe2019attention} distinguished between faithful and plausible explanations and introduced several diagnostic tools. 
%One of their tests ({\it diagnosing attention distributions by guiding simpler models}, in their  \S3.4) has similarities with the relation between the explainer and the layperson proposed in our work. 
%\citet{jain2019attention} claims attention is not explanation by comparing attention mappings to gradient probing information. \citet{serrano2019attention} proposes a ablation strategy that eliminates one feature at the time looking for decision shifts, concluding that attention is not a fail-safe indicator. \citet{wiegreffe2019attention} questions the conclusions of \citet{jain2019attention} and proposes various explainability tests. 
%These works, however, resort to analyzing attention-based methods, and 
\citet{mullenbach-etal-2018-explainable}  use human evaluation to show that attention mechanisms produce plausible explanations, consistent with our findings in \S\ref{sec:human_evaluation}. 
None of these works, however, considered the sparse selective attention mechanisms  proposed in \S\ref{sec:attention}. 
%Our goal is not to distinguish between faithful and plausible explanations. In contrast, we focus on better characterizing when explanations should be considered plausible, by providing a framework that gives an objective answer to this question. 
%As discussed in \citet[\S5]{wiegreffe2019attention}, plausible explanations are very important even if not faithful: \citet{rudin2019stop} defines explainability as a plausible reconstruction of the decision-making process, and \citet{riedl2019human} argues that they mimic what humans do when rationalizing past actions. 
Hard stochastic attention has been considered by  \citet{xu2015show,lei2016rationalizing,alvarez2017causal,bastings2019interpretable}, but a  comparison with sparse attention and explanation strategies was still missing. 


%\andre{we may need to justify somewhere why we don't follow their proposal of examining the prediction power of attention distributions in a ‘clean’ setting, where the trained parts of the model have no access to neighboring tokens of the instance.} 

Besides attention-based methods, 
many other explainers have been proposed using gradients \citep{bach2015pixel,Montavon2018,ding-etal-2019-saliency}, %\citep{bach2015pixel}, DeepLIFT \citep{shrikumar2017learning} and Integrated Gradients \citep{sundararajan2016gradients}, 
leave-one-out strategies \citep{feng2018pathologies,serrano2019attention}, 
or local perturbations  \citep{ribeiro2016should,Koh2017}, but a link with filters and wrappers in the  feature selection literature has never been made. 
%\andre{Methods that produce a measure of importance by looking to the \textbf{gradients} of the classifier output with respect to each input $\partial \hat{y} / \partial x_i$ can be considered as a form of post-hoc explanation. Another possibility is to use gradients to look the contribution of neurons in previous layers to the output. Example of methods that rely on the idea of looking at the gradients inside a neural network are Layer-wise Relevance Propagation \citep{bach2015pixel}, DeepLIFT \citep{shrikumar2017learning} and Integrated Gradients \citep{sundararajan2016gradients}. In this case, the explainer could pick the top-k words whose gradients have the largest magnitude, retrieving them as $m$. This scenario is similar to the gradient based ranking of attention weights performed by \citep{jain2019attention,wiegreffe2019attention,serrano2019attention}.}
% \andre{can you trim this paragraph? these methods are not very relevant for our paper.} 
% Inside the class of post-hoc explainers we also have perturbation methods, which analyze the impact of the classifier output with respect to perturbations to the input. An example of such method is LIME \citep{ribeiro2016should}, which extracts explanations by generating local perturbations on the input features and measuring their impact with a simple linear model. Other examples of perturbation explainers are Influence Functions \citep{Koh2017} and Shapley Values \citep{Lundberg2017}. For example, perturbations in form of feature removals were used by \citet{jain2019attention} in their leave-one-out experiments to access attention faithfulness. We consider all these as wrapper methods, since they require multiple calls to the classifier.
%Inside the class of post-hoc explainers we also have perturbation methods, 
% which analyze the impact of the classifier output with respect to perturbations to the input. An example of 
%such as LIME \citep{ribeiro2016should}, 
% which extracts explanations by generating local perturbations on the input features and measuring their impact with a simple linear model. Other examples of perturbation explainers are 
%and Influence Functions \citep{Koh2017}.
% and Shapley Values \citep{Lundberg2017}. 
%For example, perturbations in form of feature removals were used by \citet{jain2019attention} in their leave-one-out experiments to access attention faithfulness. We consider all these as wrapper methods, since they require multiple calls to the classifier. 
We believe the connections revealed in  \S\ref{sec:feature_selection} may be useful to develop new explainers in the future.

Our trained explainers from \S\ref{subsec:joint_e_and_l} draw inspiration from emergent communication \citep{lazaridou2016multi,foerster2016learning,havrylov2017emergence}. Some of our proposed ideas (e.g., using sparsemax for end-to-end differentiability) may also be relevant to that task. 
Our work is also related to sparse auto-encoders, which seek sparse overcomplete vector representations to improve model interpretability \citep{faruqui2015sparse,trifonov2018learning,subramanian2018spine}. 
In contrast to these works, we consider the non-zero attention probabilities as a form of explanation. 


Some recent work \citep{yu2019rethinking,deyoung2019eraser} advocates {\it comprehensive} rationales. 
While comprehensiveness could be useful in our framework to prevent trivial communication protocols between the explainer and layperson, 
we argue that it is not always a desirable property, since it leads to longer explanations and an increase of human cognitive load. In fact, our analysis of CSR as a function of message length (Figure~\ref{fig:k_analysis}) suggests that shorter explanations might be preferable. This is aligned to the ``explanation selection'' principle articulated by \citet[\S 4]{miller2019explanation}: {\it ``Similar to causal connection, people do not typically provide all causes for an event
as an explanation. Instead, they select what they believe are the most relevant causes.''}
Our sparse, selective attention mechanisms proposed in \S\ref{sec:attention} are inspired by this principle.  
%\andre{Hilton [70] argues that explanation selection is used for cognitive reasons: causal chains
%are often too large to comprehend. He provides an example [70, p. 43, Figure 7] showing the causal chain for the story of the fatal car accident involving ‘Mr. Jones’ from
%Kahneman and Tversky [83]. For a simple story of a few paragraphs, the causal chain
%consists of over 20 events and 30 causes, all relevant to the accident. However, only a
%small amount of these are selected as explanations [172].''}


%\andre{maybe mention also how our work relates to distillation}
%\marcos{What are the differences to distillation? 
%1. In distillation the main goal is to produce a classifier $C_2$ with less parameters, which is not necessarily simple, in fact, it still can be very complex (e.g.distill bert). 
%2. In distillation the interesting part is for $C_2$ to achieve a high performance when it is given the whole input, and not a subset of words (the message in our framework).}


%Yet, these approaches are orthogonal to ours and both may benefit from each other.

\begin{comment}
Finally, \citet{jain2020learning} proposed binarization heuristics to derive discrete rationales from gradient and attention-based explainers. While their method bears similarities with our classifier-explainer-layperson framework, there are important differences: they use the component that in our case is the layperson as their final classifier, while we use it instrumentally in a forward simulation setting. The CSR metric is absent from their work, and so is the selective sparse attention and the joint explainer-layperson. Note, however, that like their work our layperson can also be used as a classifier 
``faithful by design.''
\end{comment}

%\andre{we may need to explain better how our work %relates to \citet{lei2016rationalizing} and have a paragraph about rationales, citing \citet{zaidan2008modeling}}


%\marcos{
%\begin{itemize}
%\item Focando em NLP, ha tambem varios trabalhos que focam rationales do texto
%\item Citar alguns desses trabalhos, falando brevemente como fazem isso
%\item Alvarez-Melis, D., Jaakkola, T. S. (2017).
%\item L. Arras, G. Montavon, K. Müller, W. Samek, Explaining recurrent neural net- work predictions in sentiment analysis, (2017)
%\item Bastings, Joost Aziz, Wilker Titov, Ivan (2019)
%\end{itemize}
%}

%\marcos{Falar sobre avaliacao humana de attention weights}

% \marcos{Mullenbach et al. (2018) and Ehsan et al. (2019)}

% \andre{que papers sao estes? é necessário referir?}
% \marcos{Deixa-me lembrar aqui}
% \marcos{This paper seems relevant: \url{https://arxiv.org/abs/1806.10758}}

% Works such as Mullenbach et al. (2018) and Ehsan et al. (2019) use human evaluation to evaluate explanations; the former based on attention scores over the input, and the latter based on systems with additional rationale-generation capability. The authors show that rationales generated in a post-hoc manner increase user trust in a system.

% Explainable prediction of medical codes from clinical text - Mullenbach et al. (2018)
% Automated rationale generation: a technique for explainable ai and its effects on human perceptions - Ehsan et al. (2019)


==> BlackBoxNLP 2020 - SCE/supp_material.tex <==
\appendix


% \section{Supplemental Material}
% \label{sec:supplemental}



\section{Sparse attention}\label{sec:supp_attention}

% \andre{need to modify below}
% An example is the {\bf sparsemax transformation} \citep{martins2016softmax}, 
A natural way to get a sparse attention distribution is by using the {\bf sparsemax transformation} \citep{martins2016softmax},
which computes an Euclidean projection of the score vector onto the probability simplex $\triangle^n := \{\mathbf{p} \in \mathbb{R}^n \mid \mathbf{p}\ge \mathbf{0}, \,\, \mathbf{1}^\top\mathbf{p} = 1\}$, or, more generally, the {\bf $\alpha$-entmax transformation} \citep{peters2019sparse}: 
    \begin{equation}\label{eq:entmax}
        \alpha\text{-entmax}(\mathbf{s}) := \argmax_{\mathbf{p} \in \triangle^{n}} \mathbf{p}^\top \mathbf{s} + H_\alpha(\mathbf{p}),
    \end{equation}
where $H_\alpha$ is a generalization of the Shannon and Gini entropies proposed by \citet{Tsallis1988},  parametrized by a scalar $\alpha\ge 1$: 
\begin{equation}\label{eq:tsallis}
    H_\alpha (\mathbf{p}) := \begin{cases}
                                                \frac{1}{\alpha(\alpha-1)}\sum_j(p_j-p_j^\alpha), &  \alpha \neq 1\\
                                                -\sum_j p_j \log p_j, & \alpha=1.
                                            \end{cases}
\end{equation}
Setting $\alpha=1$ recovers the softmax function, while for any value of $\alpha>1$ this transformation can return a sparse probability vector. %(as the value of $\alpha$ increases, the induced probability distribution becomes more sparse). 
Letting $\alpha=2$, we recover sparsemax. A popular choice is $\alpha=1.5$, which has been successfully used  in machine translation and morphological inflection applications \citep{peters2019sparse}.


\section{Data statistics and preparation} \label{sec:data_statistics_preparations}

% We picked the same datasets as \citet{jain2019attention} and \citet{wiegreffe2019attention}, excluding the smallest ones. Like them, for AgNews, we considered the binary case of World vs Business articles. 
We used four datasets for text classification:  
SST,\footnote{\url{https://nlp.stanford.edu/sentiment/}} 
IMDB,\footnote{\url{https://ai.stanford.edu/~amaas/data/sentiment/}}
AgNews,\footnote{\url{https://www.di.unipi.it/~gulli/AG_corpus_of_news_articles.html}} 
and Yelp.\footnote{\url{https://www.yelp.com/dataset/}}
One dataset for NLI:
SNLI,\footnote{\url{https://nlp.stanford.edu/projects/snli/}} along with its extended version (eSNLI\footnote{\url{https://github.com/OanaMariaCamburu/e-SNLI}}) which includes human-annotated explanations of the entailment relations \citep{esnli2018}. And the EN$\to$DE IWSLT 2017 dataset for machine translation \citep{cettolo2017overview}.\footnote{\url{https://wit3.fbk.eu/mt.php?release=2017-01-trnted}} Table~\ref{table:datasets} shows statistics for each dataset.

\begin{table}[!htb]
    \small
    \begin{center}
    \begin{tabular}{lcccc}
        \toprule
        \sc Name & \sc \# Train & \sc \# Test & \sc Avg. tokens & \sc \# Classes \\
        \midrule
        SST         & 6920          & 1821          & 19          & 2 \\
        IMDB        & 25K           & 25K           & 280         & 2 \\
        AgNews     & 115K          & 20K           & 38          & 2 \\
        Yelp        & 5.6M          & 1M            & 130         & 5 \\
        SNLI        & 549K          & 9824          & 14 / 8      & 3 \\
        % MNLI        & 392K          & 20K         & 22          & 3 \\
        %eSNLI       & 549K          & 9824          & 14 / 8      & 3 \\
        IWSLT       & 206K          & 2271          & 20 / 18     & 134,086  \\
        % source vocab size: 58728       
        % target vocab size: 134086
        \bottomrule
    \end{tabular}
    \end{center}
    \caption{Dataset statistics. The average number of tokens for SNLI is related to the premise and hypothesis, and for IWSLT to the source and target sentences.} 
    \label{table:datasets}
\end{table}

For AgNews, we considered the binary case of World vs Business articles. Although the selected datasets are the same as in previous works \citep{jain2019attention,wiegreffe2019attention}, the training and test set might differ. For SST, IMDB, IWSLT and SNLI  we used the standard splits, but for AgNews and Yelp we randomly split the dataset, leaving 85\% for training and 15\% for test. 
Moreover, for IMDB, AgNews and Yelp we randomly selected 10\%, 15\% and 15\% of examples from the training set to be used as validation data, respectively. 


\section{Computing infrastructure}

Our infrastructure consists of 4 machines with the specifications shown in Table~\ref{table:computing_infrastructure}. The machines were used interchangeably, and all experiments were executed in a single GPU. Despite having machines with different specifications, we did not observe large differences in the execution time of our models across different machines. 
% Furthermore, all of our models fit in a single GPU. 

\begin{table}[!htb]
    \small
    \begin{center}
    \begin{tabular}{l ll}
        \toprule
        \sc \# & \sc GPU & \sc CPU  \\
        \midrule
        % hermes
        1.   & 4 $\times$ Titan Xp - 12GB           & 16 $\times$ AMD Ryzen 1950X @ 3.40GHz - 128GB \\
        % athena
        2.   & 4 $\times$ GTX 1080 Ti - 12GB        & 8 $\times$ Intel i7-9800X @ 3.80GHz - 128GB \\
        % zeus
        3.   & 3 $\times$ RTX 2080 Ti - 12GB        & 12 $\times$ AMD Ryzen 2920X @ 3.50GHz - 128GB \\
        % hera
        4.   & 3 $\times$ RTX 2080 Ti - 12GB        & 12 $\times$ AMD Ryzen 2920X @ 3.50GHz - 128GB \\
        \bottomrule
    \end{tabular}
    \end{center}
    \caption{Computing infrastructure.} 
    \label{table:computing_infrastructure}
\end{table}





\section{Classifiers experimental setup (Table~\ref{table:results_classifiers})} \label{sec:training_details}

We chose our classifiers so that they are close to the models used by related works \citep{jain2019attention,wiegreffe2019attention,bastings2019interpretable}. For all models, we calculated their accuracy on the dev set after each epoch. At the end of training we selected the model with the best validation accuracy. We experimented with two classes of classifiers: a simple RNN with attention as in \citet{jain2019attention,wiegreffe2019attention}; and the rationalizer models of \citet{lei2016rationalizing} and \citet{bastings2019interpretable} which sample binary masks from Bernoulli and HardKuma distributions, respectively. 

\subsection{RNNs with attention} \label{subsec:rnns_with_attn}
For the text classification experiments, each input word $x_i$ is mapped to 300D-pretrained GloVe embeddings \citep{pennington2014glove} from the 840B release,\footnote{\url{http://nlp.stanford.edu/data/glove.840B.300d.zip}} kept frozen, followed by a bidirectional LSTM layer (BiLSTM) resulting in vectors $\mathbf{h}_1,\ldots,\mathbf{h}_n$. 
We score each of these vectors using the additive formulation of \citet{Bahdanau2015}, applying an attention transformation to convert the resulting scores $\mathbf{s} \in \mathbb{R}^n$ to a probability distribution $\pi \in \triangle^n$. 
We use this to compute a  contextual vector $\mathbf{c} = \sum_{i=1}^n \pi_i \mathbf{h_i}$, which  is  fed into the output softmax layer that predicts $\hat{y}$. 
For NLI, the input $x$ is a pair of sentences (a premise and an hypothesis), and the classifier $C$ is similar to the the above, but with two independent BiLSTM layers, one for each sentence. In the attention layer, we use the last hidden state of the hypothesis as the query and the premise vectors as keys. 

We used the AdamW \cite{loshchilov2018decoupled} optimizer for all experiments. We tuned two hyperparameters: learning rate within $\{0.003, \mathbf{0.001}, 0.0001\}$, and $l_2$ regularization within $\{0.01, 0.001, \mathbf{0.0001}, 0\}$. We picked the best configuration by doing a grid search and by taking into consideration the accuracy on the validation set (selected values in bold).  Table~\ref{tab:table_all_hyperparams_rnns} shows all hyperparameters set for training. 


\begin{table}[!htb]
    \centering
    \small
    \begin{tabular}{llllll}
    \toprule
    \sc Hyperparam.             & \sc SST & \sc IMDB & \sc AgNews & \sc Yelp &  \sc SNLI \\
    \midrule
    Word embeddings size        & 300   & 300   & 300   & 300   & 300      \\
    BiLSTM hidden size          & 128   & 128   & 128   & 128   & 128     \\
    Merge BiLSTM states         & concat    & concat    & concat    & concat    & concat \\
    
    Batch size                  & 8     & 16    & 16    & 128   & 32      \\
    Number of epochs            & 10    & 10    & 5     & 5    & 10    \\
    Early stopping patience     & 5     & 5     & 3     & 3     & 5     \\
    Learning rate               & 0.001     & 0.001     & 0.001     & 0.001     & 0.001     \\
    $\ell_2$ regularization     & 0.0001    & 0.0001    & 0.0001    & 0.0001    & 0.0001     \\
    \bottomrule
    \end{tabular}
    \caption{RNNs training hyperparameters for text classification and NLI datasets.}
    \label{tab:table_all_hyperparams_rnns}
\end{table}


\subsection{Bernoulli and HardKuma} \label{subsec:bernolli_and_hardkuma}

We used the implementation of \citet{bastings2019interpretable},\footnote{\url{https://github.com/bastings/interpretable_predictions}} which includes a reimplementation of the generator-encoder model from \citep{lei2016rationalizing}.
The model used for text classification is a RNN-based generator followed by a RNN-based encoder, whereas for NLI is a decomposable attention classifier from \citep{parikh-etal-2016-decomposable}, for which only the HardKuma implementation was available. 
In order to faithfully compare the frameworks, we adapted the HardKuma code and implemented a Bernoulli version of the same classifier, taking into consideration the sparsity and fused-lasso loss penalties, and the deterministic strategy used during test time. For simplicity, we used the independent variant of the generator of \citet{lei2016rationalizing}.
Table~\ref{tab:table_all_hyperparams_rationalizing} lists only the hyperparameters that we set during training. We refer to the original work of \citet{bastings2019interpretable} to see all other hyperparamers, for which we kept the default values.

\begin{table}[!htb]
    \centering
    \small
    \begin{tabular}{llllll}
    \toprule
    \sc Hyperparam.                 & \sc SST & \sc IMDB & \sc AgNews & \sc Yelp &  \sc SNLI \\
    \midrule
    % Latent selection (HardKuma)     & 0.3       & 0.3       & 0.3       & 0.3       & 0.1      \\
    % Sparsity penalty (Bernoulli)    & 0.01      & 0.0003    & 0.01      & 0.01      & 0.0003      \\
    Latent selection (HardKuma)     & 0.3       & 0.1       & 0.3       & 0.3       & 0.1      \\
    Sparsity penalty (Bernoulli)    & 0.01      & 0.001     & 0.01      & 0.01      & 0.0003      \\
    
    Lasso penalty    & 0        & 0     & 0      & 0      & 0      \\
    
    Batch size                      & 25        & 25        & 25        & 256       & 64     \\
    Number of epochs                & 25        & 25        & 25        & 10        & 100    \\
    Early stopping patience         & 5         & 5         & 5         & 5         & 100    \\
    Learning rate                   & 0.0002    & 0.0002    & 0.0002    & 0.001     & 0.0002     \\
    $\ell_2$ regularization         & $10^{-5}$ & $10^{-5}$ & $10^{-5}$ & $10^{-5}$ & $10^{-6}$     \\
    \bottomrule
    \end{tabular}
    \caption{Rationalizer models training hyperparameters for text classification and NLI datasets.}
    \label{tab:table_all_hyperparams_rationalizing}
\end{table}


\subsection{Validation set results and model statistics}

Table~\ref{table:classifiers_statistics_params} shows the accuracy of each classifier on the validation set, their number of trainable parameters and the average training time per epoch.

% \begin{table*}[!htb]
% \scriptsize
% \begin{center}
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{l ccc c ccc c ccc c ccc c ccc}
% \toprule
% & \multicolumn{3}{c}{\sc SST} & & \multicolumn{3}{c}{\sc IMDB} & & \multicolumn{3}{c}{\sc AgNews} & & \multicolumn{3}{c}{\sc Yelp} & & \multicolumn{3}{c}{\sc SNLI} \\


% \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}  \cmidrule{18-20} 

% \sc Clf.\,\, & 
% \sc \# P & \sc $t$ & \sc ACC  & & 
% \sc \# P & \sc $t$ & \sc ACC  & & 
% \sc \# P & \sc $t$ & \sc ACC  & & 
% \sc \# P & \sc $t$ & \sc ACC  & & 
% \sc \# P & \sc $t$ & \sc ACC  \\

% \midrule 

% $C$                 & 474K & 10s & 00.00    & & 474K & 2m & 00.00     & & 474K & 2m & 00.00     & & 474K & 3h & 00.00     & & 998K & 4m & 00.00 \\
% $C_{\text{sp}}$     & 474K & 10s & 00.00    & & 474K & 2m & 00.00     & & 474K & 2m & 00.00     & & 474K & 3h & 00.00     & & 998K & 4m & 00.00 \\
% $C_{\text{ent}}$    & 474K & 10s & 00.00    & & 474K & 2m & 00.00     & & 474K & 2m & 00.00     & & 474K & 3h & 00.00     & & 998K & 4m & 00.00 \\
% $C_{\text{bern}}$   & 1.1M & 15s & 00.00    & & 1.1M & 2m & 00.00     & & 1.1M & 2m & 00.00     & & 1.1M & 5h & 00.00     & & 382K & 2m & 00.00 \\
% $C_{\text{hk}}$     & 1.1M & 15s & 00.00    & & 1.1M & 2m & 00.00     & & 1.1M & 2m & 00.00     & & 1.1M & 5h & 00.00     & & 462K & 2m & 00.00 \\

% \bottomrule
% \end{tabular}
% % }
% \end{center}
% \caption{Classifier results on the validation set and model statistics. \# P is the number of trainable parameters, and is $t$ the average run time per epoch.} 

% \label{table:classifiers_statistics_params}

% \end{table*}

\begin{table*}[!htb]
\small
\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l ccc c ccc c ccc}
\toprule
& \multicolumn{3}{c}{\sc SST} & & \multicolumn{3}{c}{\sc IMDB} & & \multicolumn{3}{c}{\sc AgNews} \\


\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}

\sc Clf.\,\, & 
\sc \# P & \sc $t$ & \sc ACC  & & 
\sc \# P & \sc $t$ & \sc ACC  & & 
\sc \# P & \sc $t$ & \sc ACC  \\

\midrule 

$C$                 & 474K & 10s & 85.32    & & 474K & 2m & 95.64     & & 474K & 2m & 98.09  \\
$C_{\text{ent}}$    & 474K & 10s & 84.29    & & 474K & 2m & 95.84     & & 474K & 2m & 98.54  \\
$C_{\text{sp}}$     & 474K & 10s & 84.17    & & 474K & 2m & 95.44     & & 474K & 2m & 98.51  \\
$C_{\text{bern}}$   & 1.1M & 15s & 80.16    & & 1.1M & 2m & 87.40     & & 1.1M & 2m & 96.26  \\
$C_{\text{hk}}$     & 1.1M & 15s & 84.40    & & 1.1M & 2m & 91.84     & & 1.1M & 2m & 96.74  \\

\bottomrule
\end{tabular}
% }
\end{center}
\caption{Classifier results on the validation set and model statistics. \# P is the number of trainable parameters, and is $t$ the average training time per epoch.} 

\label{table:classifiers_statistics_params}

\end{table*}




\begin{table*}[!htb]
\small
\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l ccc c ccc}
\toprule
& \multicolumn{3}{c}{\sc Yelp} & & \multicolumn{3}{c}{\sc SNLI} \\


\cmidrule{2-4} \cmidrule{6-8}

\sc Clf.\,\, & 
\sc \# P & \sc $t$ & \sc ACC  & & 
\sc \# P & \sc $t$ & \sc ACC  \\

\midrule 

$C$                 & 474K & 3h & 77.03     & & 998K & 4m & 78.74 \\
$C_{\text{ent}}$    & 474K & 3h & 76.72     & & 998K & 4m & 79.38 \\
$C_{\text{sp}}$     & 474K & 3h & 76.84     & & 998K & 4m & 79.69 \\
$C_{\text{bern}}$   & 1.1M & 5h & 69.99     & & 382K & 2m & 79.79 \\
$C_{\text{hk}}$     & 1.1M & 5h & 74.29     & & 462K & 2m & 86.04 \\

\bottomrule
\end{tabular}
% }
\end{center}
\caption{Continuation of Table~\ref{table:classifiers_statistics_params}.} 

\label{table:classifiers_statistics_params_2}

\end{table*}



\section{Communication experimental setup (Table~\ref{table:results_doc_classification})} \label{sec:communication_details}

Training the communication under our framework consists on training a layperson $L$ on top of explanations (message) produced by $E$ about $C$'s decision. With the exception of the explainer $E$ trained jointly with $L$, none of the other explainers have trainable parameters. Therefore, in these cases, the communication between $E$ and $L$ consists only on training $L$. For all models, we calculated its CSR on the dev set after each epoch. At the end of training we selected the model with the best validation CSR. Table~\ref{tab:table_all_hyperparams_comm} shows the communication hyperparameters. Note that for SNLI we still need to train a BiLSTM to encode the hypothesis.

\begin{table}[!htb]
    \centering
    \small
    \begin{tabular}{llllll}
    \toprule
    \sc Hyperparam.             & \sc SST & \sc IMDB & \sc AgNews & \sc Yelp &  \sc SNLI \\
    \midrule
    Word embeddings size        & -   & -   & -   & -   & 300      \\
    BiLSTM hidden size          & -   & -   & -   & -   & 128     \\
    Merge BiLSTM states         & -   & -   & -   & -   & concat \\
    
    Batch size                  & 16    & 16    & 16    & 112   & 64      \\
    Number of epochs            & 10    & 10    & 10    & 5     & 10    \\
    Early stopping patience     & 3     & 3     & 3     & 3     & 3     \\
    Learning rate               & 0.001 & 0.001 & 0.001 & 0.003 & 0.001     \\
    $\ell_2$ regularization     & $10^{-5}$ & $10^{-5}$ & $10^{-5}$ & $10^{-5}$ & $10^{-5}$     \\
    \bottomrule
    \end{tabular}
    \caption{Communication hyperparameters for text classification and NLI datasets.}
    \label{tab:table_all_hyperparams_comm}
\end{table}


\subsection{Validation set results and model statistics}

Table~\ref{table:communication_statistics_params} shows the CSR and ACC$_L$ for each explainer on the validation set, the number of trainable parameters of $L$ and the average training time per epoch.

\begin{table*}[!htb]
\small
\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l cccc c cccc c cccc}
\toprule
& \multicolumn{4}{c}{\sc SST} & & \multicolumn{4}{c}{\sc IMDB} & & \multicolumn{4}{c}{\sc AgNews}\\


\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15}

\sc Explainer\,\, & 
\sc \# P & \sc $t$ & CSR & ACC$_L$  & & 
\sc \# P & \sc $t$ & CSR & ACC$_L$  & & 
\sc \# P & \sc $t$ & CSR & ACC$_L$  \\

\midrule 

Random                  & 38K & 10s & 63.76 & 62.84   & & 247K & 1m & 61.36 & 61.24    & & 120K & 2m & 85.26 & 84.58 \\
Erasure                 & 38K & 10s & 81.88 & 79.82   & & 247K & 2m & 94.00 & 91.40    & & 120K & 3m & 98.41 & 96.98 \\
Top-$k$ gradient        & 38K & 10s & 76.72 & 75.57   & & 247K & 1m & 91.88 & 89.52    & & 120K & 2m & 98.23 & 96.97 \\

Top-$k$ softmax         & 38K & 20s & 84.29 & 80.62   & & 247K & 1m & 96.60 & 93.60    & & 120K & 2m & 98.54 & 97.14 \\
Top-$k$ 1.5-entmax      & 38K & 20s & 85.44 & 80.28   & & 247K & 1m & 97.88 & 94.92    & & 120K & 2m & 98.22 & 97.37 \\
Top-$k$ sparsemax       & 38K & 20s & 85.44 & 81.54   & & 247K & 1m & 96.76 & 93.32    & & 120K & 2m & 96.46 & 95.72 \\

Select. 1.5-entmax      & 38K & 10s & 85.55 & 80.62   & & 247K & 1m & 97.44 & 94.56    & & 120K & 1m & 98.30 & 97.41 \\
Select. sparsemax       & 38K & 10s & 85.44 & 81.54   & & 247K & 1m & 97.04 & 93.36    & & 120K & 1m & 96.46 & 95.72 \\

Bernoulli               & 38K & 5s & 84.75 & 78.21   & & 247K & 1m & 91.80 & 87.36    & & 120K & 1m & 97.12 & 94.82 \\
HardKuma                & 38K & 5s & 87.50 & 81.76   & & 247K & 1m & 95.36 & 91.20    & & 120K & 1m & 97.38 & 96.05 \\
% 54:40
\bottomrule
\end{tabular}
% }
\end{center}
\caption{Communication results on the validation set and explainer statistics. \# P is the number of trainable parameters, and is $t$ the average training time per epoch.} 

\label{table:communication_statistics_params}

\end{table*}





\begin{table*}[!htb]
\small
\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l cccc c cccc}
\toprule
& \multicolumn{4}{c}{\sc Yelp} & & \multicolumn{4}{c}{\sc SNLI} \\


\cmidrule{2-5} \cmidrule{7-10}

\sc Explainer\,\, & 
\sc \# P & \sc $t$ & CSR & ACC$_L$  & & 
\sc \# P & \sc $t$ & CSR & ACC$_L$  \\

\midrule 

Random                  & 1.8M & 3h & 52.55 & 48.21     & & 560K & 9m  & 31.04 & 33.11 \\
Erasure                 & 1.8M & 4h & 79.63 & 69.59     & & 560K & 10m & 78.72 & 70.60 \\
Top-$k$ gradient        & 1.8M & 3h & 71.81 & 63.59     & & 560K & 10m & 77.55 & 69.41 \\
Top-$k$ softmax         & 1.8M & 3h & 81.49 & 70.67     & & 560K & 9m & 79.10 & 70.95 \\
Top-$k$ 1.5-entmax      & 1.8M & 3h & 82.80 & 71.31     & & 560K & 9m & 80.30 & 73.57 \\
Top-$k$ sparsemax       & 1.8M & 3h & 82.97 & 71.46     & & 560K & 9m & 83.25 & 75.34 \\
Select. 1.5-entmax      & 1.8M & 2h & 82.90 & 70.99     & & 560K & 6m & 77.46 & 71.66 \\
Select. sparsemax       & 1.8M & 2h & 84.67 & 72.25     & & 560K & 6m & 82.33 & 75.11 \\

Bernoulli               & 1.8M & 2h & 84.93 & 66.77     & & 560K & 2m & 75.75 & 68.61 \\
HardKuma                & 1.8M & 2h & 87.43 & 71.57     & & 560K & 3m & 75.10 & 71.10 \\
% 21:10
\bottomrule
\end{tabular}
% }
\end{center}
\caption{Continuation of Table~\ref{table:communication_statistics_params}.} 

\label{table:communication_statistics_params_2}

\end{table*}







\section{Joint $E$ and $L$ setup}


\subsection{Communication}

According to \S\ref{subsec:joint_e_and_l}, in this model we have two set of parameters to train, one for the explainer $E$ and other for the layperson $L$, whereas the classifier is a frozen model that we want to explain. Here, we set $C$ as the RNN with softmax classifier (see \S\ref{table:results_classifiers}). We design $E$ with the same architecture of the RNNs with attention from \S\ref{subsec:rnns_with_attn} but without a final output layer, and $L$ have the same architecture as the laypersons in \S\ref{sec:experiments}. In short, the architecture of $E$  is composed of: (i) embedding layer; (ii) BiLSTM; (iii) attention mechanism. As before, the message is constructed with the words extracted from the attention mechanism. 

We use sparsemax attention during training to ensure end-to-end differentiability, and we recover the top-$k$ attended words during test time. We used $k=5$ for IMDB and $k=4$ for SNLI in all experiments. In order to encourage faithful explanations, we set $h = \frac{1}{L}\sum_i C_{\mathrm{RNN}}(x_i)$ and $\tilde{h} = \frac{1}{L}\sum_i \mathrm{FFN}(E_{\mathrm{RNN}}(x_i))$, where $\mathrm{FFN}$ is a simple feed-forward layer, and $C_{\mathrm{RNN}}(x_i)$ and $E_{\mathrm{RNN}}(x_i)$ are the BiLSTM states from the classifier and the explainer, respectively. In other words, we are approximating the average of the BiLSTM states of $C$ and $E$. We set $\lambda=1$ and $\beta=0.2$ and used the same hyperparameters as in Table~\ref{tab:table_all_hyperparams_comm}. 
The list of stopwords used in our experiments contains 127 English words extracted from NLTK.
%\marcos{say something about testing different values of $\lambda$?}



\subsection{Analysis of $\beta$}\label{sec:analysis_beta}

% \paragraph{Quality of the explanations.} 

A potential problem of this model is for the two agents to agree on a trivial protocol, ensuring a high CSR even with bad quality explanations (e.g. punctuations or stopwords). Besides preventing stopwords to be in the message,\footnote{In practice, we simply set attention scores associated with stopwords to $-\infty$.} we set a different probability $\beta$ of the explainer accessing the predictions of the classifier $\hat{y}$. Intuitively, these strategies should encourage explanations to have higher quality. One way to quantitatively access the quality of the explanations is by aggregating the  relative frequencies of each selected word in the validation set, and calculating its Shannon's entropy. If the entropy is low, then the  explanations have a high number of repetitions and the explainers are focusing on a very small subset of words, denoting a trivial protocol. To check for a reasonable entropy score that resembles a good quality explanation, we investigate the entropy of the other explainers, for which we had confirmed their quality via human evaluation. 
% Table~\ref{tab:entropy_explainers} shows the entropy of each explainer on IMDB and SNLI.

In order to see the impact of $\beta$, we carried an experiment with increasing values of $\beta$ and looked at the CSR, ACC$_L$ and the entropy ($H$) of the generated explanations. Results are shown in Table~\ref{tab:results_joint_betas} for each explainer on IMDB and SNLI.

\begin{table}[!htb]
\small
\begin{center}
\begin{tabular}{ll ccc@{ }c ccc@{ }c}
\toprule
& & \multicolumn{3}{c}{\sc IMDB} & & \multicolumn{3}{c}{\sc SNLI} \\


\cmidrule{3-5} \cmidrule{7-9} 

\sc Clf. & \multirow{1}{*}{\sc Explainer} & $H$ & CSR & ACC$_L$  & & $H$ & CSR & ACC$_L$ \\
% Note: the CSR and ACC of these explainers are different from table 4 for IMDB because here we used k=5 (instead of k=10)
\midrule 
$C$         & Random                  & 9.13 & 59.20 & 58.92 		& & 8.21 & 31.04 & 33.11     \\
$C$         & Erasure                 & 9.40 & 96.32 & 93.48 		& & 9.75 & 78.72 & 70.60     \\
$C$         & Top-$k$ gradient        & 9.49 & 85.84 & 83.72 		& & 9.39 & 77.55 & 69.41     \\
$C$         & Top-$k$ softmax         & 9.38 & 94.44 & 91.84 		& & 9.76 & 78.66 & 71.00     \\
$C_{ent}$   & Top-$k$ 1.5-entmax      & 9.62 & 95.20 & 93.36 		& & 9.54 & 80.30 & 73.57     \\
$C_{sp}$    & Top-$k$ sparsemax       & 9.56 & 95.28 & 92.56 		& & 8.79 & 83.25 & 75.34     \\

$C_{ent}$   & Select. 1.5-entmax      & 10.76 & 97.44 & 94.56 		& & 8.49 & 77.46 & 71.66     \\
$C_{sp}$    & Selec. sparsemax        & 10.41 & 97.04 & 93.36 		& & 8.38 & 82.33 & 75.11     \\
% $C_{bern}$  & Bernoulli               & 9.61 & 91.60 & 87.36 		& & 8.27 & 75.65 & 68.68     \\
% $C_{hk}$    & HardKuma                & 11.54 & 94.20 & 90.80 		& & 9.93 & 71.57 & 68.30     \\
$C_{bern}$  & Bernoulli               & 10.66 & 91.88 & 87.36 		& & 8.27 & 75.75 & 68.61     \\
$C_{hk}$    & HardKuma                & 11.38 & 95.36 & 91.20 		& & 9.93 & 75.10 & 71.10     \\


-           & Human highlights        & -     & -     & - 		    & & 8.72 & 87.97 & 87.97     \\
\midrule 
$C$         & Joint $E$ and $L$ ($\beta=0.0$)        & 6.16 & 93.04 & 90.84   	& & 9.81 & 80.74 & 72.38  \\
$C$         & Joint $E$ and $L$ ($\beta=0.2$)	     & 6.05 & 98.52 & 94.56   	& & 9.81 & 93.44 & 77.20  \\
$C$         & Joint $E$ and $L$ ($\beta=0.5$)	     & 5.63 & 99.68 & 95.64   	& & 9.45 & 95.81 & 77.54  \\
$C$         & Joint $E$ and $L$ ($\beta=1.0$)	     & 3.72 & 99.92 & 95.56   	& & 9.01 & 97.49 & 77.23  \\

\bottomrule
\end{tabular}
\end{center}
\caption{Entropy of the explanations for all explainers on the validation set of IMDB and SNLI. Entropy for human highlights was calculated based on non-neutral examples. 
% $C_\star$ represents a classifier with a 100\% accuracy.
% Explanations for top-$k$ explainers were extracted using $k=5$.
% $S$ denotes the entropy of the explanations.
} 
\label{tab:results_joint_betas}
\end{table}

When $\beta=0$ no information about the label predicted by the classifier is being exposed to the explainer, and as a result we have a model that resembles a combination of selective (during training) and top-$k$ (during test time) sparsemax explainers. This means that the results between these explainers are expected to be very similar in terms of CSR.\footnote{Note that this also depends on the performance of $C$ and $C_{sp}$, which are indeed very similar in this case: 95.64 and 95.44.} Overall, for both datasets, we can see a tradeoff between CSR and entropy $H$ as $\beta$ increases, suggesting that CSR is not able to capture the notion of quality (which was expected due to the subjective nature of an explanation). For IMDB the entropy values were lower than our previous explainers, but for SNLI they were very similar. A potential reason for this is the particularity of the two datasets: IMDB have long documents (280 words on average) with a large set of repetitive words which are not stopwords and are strongly correlated with the labels (e.g. good, ok, bad, etc.); SNLI premises are very short (14 words on average) without a large set of repetitive words.
Finally, due to this tradeoff, we selected $\beta=0.2$ for all of our experiments since it induces a very high CSR with a reasonably good entropy.


\begin{comment}
\paragraph{Degeneration problem.} The problem we call \aspas{trivial protocol} has been diagnosed by \citet{yu2019rethinking} as \aspas{degeneration problem}. Their strategy was to use the notion of comprehensiveness to penalize the predictive power of a classifier trained on the complement set of the selected explanations (i.e. the words that were not selected by the explainer) \marcos{check. Andre can you check this? I'm not sure if they are minimizing or maximizing the entropy of the complement set.}. In contrast, we follow the selective explanation principle of \citet{miller2019explanation} and focus on \textit{sufficient} rationales, adopting a much simpler strategy where we can control the amount of \aspas{degeneration} by carefully setting $\beta$, and selecting the final model by looking at the entropy of the explanations.
\end{comment}



\section{Machine Translation experiments}\label{sec:nmt_setup}


\subsection{Data}

To compare explainers on a more challenging task with large $|\mathcal{Y}|$, we ran an experiment on neural machine translation (NMT), adapting the JoeyNMT framework \citep{kreutzer2019joey}. 
We used the EN$\to$DE IWSLT 2017 dataset \citep{cettolo2017overview}, with the standard splits (Table~\ref{table:datasets}). %We replicated \citet{peters2019sparse} using raw words as input instead of byte-pair encodings. 

\subsection{Classifier} 

We replicated the work of \citet{peters2019sparse} with the exception that we used raw words as input instead of byte-pair encodings. The implementation is based on Joey-NMT \citep{kreutzer2019joey}. 
We employed beam search decoding with beam size of 5, achieving a BLEU score of 20.49, 21.12 and 20.75 for softmax ($C$), 1.5-entmax ($C_{\text{ent}}$) and sparsemax ($C_{\text{sp}}$), respectively. %These values are very close ($<$1.5) to the BLEU scores found in the original work of \citet{peters2019sparse}.$. 
We refer to the work of \citet{peters2019sparse} for more training details. Table~\ref{tab:table_all_hyperparams_nmt} shows the classifier hyperparameters.

% We used the default configuration file from JoeyNMT,\footnote{\url{https://github.com/joeynmt/joeynmt/blob/master/configs/iwslt14_deen_bpe.yaml}} with the following hyperpameters:

\begin{table}[!htb]
    \centering
    \small
    \begin{tabular}{ll}
        \toprule
        \sc Hyperparam. & \sc Value  \\
        \midrule
        Word embeddings size        & 512     \\
        BiRNN hidden size           & 512     \\
        Attention scorer            & \citep{Bahdanau2015} \\
        
        Batch size                  & 32    \\
        Optimizer                   & Adam      \\
        Number of epochs            & 100     \\
        Early stopping patience     & 8 \\
        Learning rate               & 0.001     \\
        % Scheduling                  & Plateau \\
        Decrease factor             & 0.5 \\
        $\ell_2$ regularization     & 0     \\
        
        RNN type                    & LSTM \\
        RNN layers                  & 2 \\
        Dropout                     & 0.3 \\
        Hidden dropout              & 0.3 \\
        % Input feeding               & True \\
        % Init. hidden                & Last \\
        
        Maximum output length & 100 \\
        Beam size & 5 \\
        \bottomrule
    \end{tabular}
    \caption{Classifier hyperparmeters for neural machine translation.}
    \label{tab:table_all_hyperparams_nmt}
\end{table}


\subsection{Communication}

We consider the decision taken by the NMT system when generating the $t^\text{th}$ target word ($y$), given the source sentence $x$ and the previously generated words $y_{1:{t-1}}$. Note that in this example $\mathcal{Y}$ is the entire target vocabulary. 
The message is the concatenation of $k$ source words (ranked by importance, without any word order information) 
% \andre{check} \marcos{what do you mean by order information?} 
% \marcos{Got it. The top k does not include the positional information of the word in the original sentence}
with the prefix $y_{1:{t-1}}$. The layperson must predict the target word given this limited information (see Fig.~\ref{fig:example_mt}). 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/mt-example-2-thick.pdf}
    \caption{Example of sparse attention for machine translation. When the model is generating the word \aspas{Veränderung}, the source words \aspas{a} and \aspas{change} are treated as explanation and sent as message.}
    % \andre{maybe underline or use a different color for the word Veranderung}
    % Done
    \label{fig:example_mt}
\end{figure}

The layperson is a model that uses an unidirectional LSTM with $256$ hidden units to encode the translation prefix, and a feed-forward layer to encode the concatenation of $k$ source word embeddings (the message) to a vector of $256$ dimensions. 
%This vector is concatenated with the output vector of the translation LSTM for the word being translated at the moment. Finally, 
The two vectors are concatenated and passed to a linear output layer to predict the next  word $\tilde{y} \in \mathcal{Y}$ from the target vocabulary. 
We used 300D-pretrained GloVe embeddings to encode source words (EN), and 300D-pretrained FastText embeddings to encode target words (DE).\footnote{\url{https://dl.fbaipublicfiles.com/fasttext/vectors-crawl/cc.de.300.bin.gz}} 
Table~\ref{tab:table_all_hyperparams_nmt_comm} shows the communication hyperparameters.

\begin{table}[!htb]
    \centering
    \small
    \begin{tabular}{ll}
        \toprule
        \sc Hyperparam. & \sc Value  \\
        \midrule

        Word embeddings size        & 300     \\
        LSTM hidden size            & 256     \\
        Merge LSTM states           & concat \\
        
        Batch size                  & 16    \\
        Number of epochs            & 10    \\
        Early stopping patience     & 5     \\
        Learning rate               & 0.003 \\
        $\ell_2$ regularization     & $10^{-5}$     \\
        \bottomrule
    \end{tabular}
    \caption{Communication hyperparmeters for neural machine translation.}
    \label{tab:table_all_hyperparams_nmt_comm}
\end{table}


\subsection{Results}

Results comparing different filtering methods varying $k$ are shown in Table~\ref{table:results_iwslt}. We show the CSR as we varied $k \in \{0,1,3,5\}$. %, meaning the scores when only the most relevant $k$ source words are shown to the layperson at each translation timestep. 
There are two main findings. First, we see again that {\bf top-$k$ attention outperforms top-$k$ gradient}, in this case with a wider margin. 
Second, we see that  all methods perform better as we increase $k$, albeit we can see a performance degradation of attention-based explainers for $k=5$. An interesting case is when $k=0$, meaning that $L$ has no access to the source sentence, behaving like an unconditioned language model. 
In this case the performance is much worse, indicating that both 
% top-$k$ attention and gradient 
explainers are selecting relevant tokens when $k>0$. %To further emphasize this claim, we trained a model which selects $k=5$ source words at random at each timestep, yielding a CSR of $23.32$, which is very close to the results when $k=0$. %As the findings described in \citep{peters2019sparse}, we also see that 1.5-entmax performs better than softmax and sparsemax.
As we found for IMDB and SNLI, as we increased $k$ we observed a trade-off between $k$ and CSR for IWSLT. Fig.~\ref{fig:k_analysis_nmt} depicts this finding.


% BLEU	    dev	        test	[Beam search decoding with beam size = 5 and alpha = 1.0]
% softmax	20.48768	20.48768	
% sparsemax	24.40572	20.74869	
% entmax15	24.52431	21.12021	



% \andre{include a figure with a real example where the explanation is important to guess the next word?}
% \marcos{I'm on it}

% \begin{itemize}
%     \item qual foi o modelo utilizado para treinar o classifier para machine translation
%     \item quais foram os hiperparametros diferentes do trabalho do Ben
%     \item qual foi o bleu score de cada metodo no conjunto de teste
%     \item como foi implementado o layperson - concat das embeddings (k * emb dim)
%     \item 
% \end{itemize}

% BLEU	    dev	        test
% softmax	20.48768	20.48768
% sparsemax	24.40572	20.74869
% entmax15	24.52431	21.12021


\begin{table}[!htb]
\small
\begin{center}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
%\multirow{2}{*}{\sc Explainer} & \multicolumn{4}{c}{CSR} \\
%\cmidrule{2-5}
\sc Clf. & \sc Explainer & $k=0$ & $k=1$ & $k=3$ & $k=5$ \\
\midrule 
% Uniform    		            & - & - & - & 23.32   	\\
% \midrule
$C$ & Top-$k$ gradient    	& 21.99     & 35.21     & 38.33     & 40.30   	\\
$C$ & Top-$k$ softmax	 	    & 21.99     & \bf 62.58 & 62.82     & 62.64   	\\
$C_{\text{ent}}$ & Top-$k$ 1.5-entmax		& \bf 22.31 & 62.53     & \bf 63.48 & \bf 62.69   	\\
$C_{\text{sp}}$ & Top-$k$ sparsemax	 	& 22.14     & 62.21     & 61.94     & 61.92   	\\
\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results for IWSLT. Reported are CSR scores.
% The classifier $C$ achieves a BLEU score of \andre{?} for this task.
% \marcos{Coloquei isso no texto acima.}
} \label{table:results_iwslt}
\end{table}




\begin{figure}[!htb]
% for now i'll let the figure this way, if I find time i'll search how to use only one legend
% it is not easy to do this and have two subfigures
    \centering
    
    % IWSLT
    % CSR plot
    \subfloat{{\input{figs/line_iwslt_csr.tex}}}
    
    \caption{Message sparsity analysis for IWSLT. For SNLI, $k=0$ corresponds to a case where the layperson only sees the translation prefix.
    The rightmost entry is the average length of the examples in the test set, and therefore it represents an explainer that simply pass forward all words to the layperson (i.e. a full bag-of-words). The average $k$ for sparsemax and 1.5-entmax are, respectively: 4.5 and 9.4.
    } \label{fig:k_analysis_nmt}
    
\end{figure}



\section{Human annotation}\label{sec:supp_interface}

% An important aspect of our framework is how it relates to human judgement. 
We had four different human annotators, two for IMDB and two for SNLI. %, who are not the authors of the paper. 
%To prevent potential knowledge bias from the annotators, the name of the explainers was anonimyzed, and to prevent easy comparison across explainers, the documents were displayed in a different order. 
No information was given about the explainers which produced each message, and documents were presented in random order. 
Since in our experiments we define the message as being a bag-of-words, which does not encode order information, the explanations (i.e. the selected words) were shuffled and displayed as a cloud of words. The annotators were asked to predict the label of each document, when seeing only these explanations. For SNLI, we show the entire hypothesis as raw text and the premise as a cloud of words. We selected top-$k$ explainers with $k=5$ for IMDB and $k=4$ for SNLI. Figure~\ref{fig:interface_attn} shows a snapshot of the annotation interface used for the experiments described in \S\ref{sec:human_evaluation}.

\begin{figure*}[!htb]
    \centering
    % \includegraphics[width=0.45\textwidth]{figs/interface-attn-nohead.png}
    \centering
    \subfloat[IMDB]{\includegraphics[width=0.37\textwidth]{figs/interface-attn-nohead.png}}
    \quad
    \subfloat[SNLI]{\includegraphics[width=0.37\textwidth]{figs/interface-attn-nohead-snli.png}}
    \caption{Snapshot of the annotation interface.}
    \label{fig:interface_attn}
\end{figure*}

By directly looking at the explanations, we observed that some of them are very ambiguous with respect to the true label, so we decided to include a checkbox to be marked in case the annotator was not sure by his/her decision. The unsure checkbox also helps to capture the notion of sufficiency, that is, if the explanations are sufficient for a human predict some label. A similar approach was employed by \citet{yu2019rethinking} using a two-stage annotation method, explicitly asking the human annotator if the rationale was sufficient for his/her decision. 
Furthermore, we calculated the agreement between explainers using the Cohen's kappa coefficient and the relative observed agreement ratio (or accuracy, $p_o$). Table~\ref{tab:table_agreement_human_eval} shows statistics for the unsure checkbox and agreement between annotators.




\begin{table}[!htb]
\small
\begin{center}

\begin{tabular}{ll ccccc c ccccc}
\toprule
\multirow{2}{*}{\sc Clf.} &
\multirow{2}{*}{\sc Explainer} & \multicolumn{5}{c}{IMDB} & & \multicolumn{5}{c}{SNLI} \\
\cmidrule{3-7}
\cmidrule{9-13}
        & & $u$ & $p_o$ & $\kappa$ & CSR$_H$ & ACC$_H$         & & $u$ & $p_o$ & $\kappa$ & CSR$_H$ & ACC$_H$ \\    
\midrule 
$C$ & Erasure 	                        & 0.05 & 0.92 & 0.83 & 89.25 & 86.25 		& & 0.25 & 0.83 & 0.66 & 72.50 & 83.50   \\
$C$ & Top-$k$ gradient 					& 0.17 & 0.76 & 0.51 & 73.50 & 73.00 	    & &	0.32 & 0.80 & 0.59 & 65.75 & 76.75    \\
$C$ & Top-$k$ softmax 					& 0.23 & 0.91 & 0.81 & 89.25 & 88.25 	    & &	0.25 & 0.78 & 0.55 & 72.00 & 82.75   \\
$C_{\text{ent}}$ & Top-$k$ 1.5-entmax 	& 0.09 & 0.91 & 0.81 & 89.25 & 85.75  	    & &	0.29 & 0.82 & 0.64 & 70.00 & 80.50   \\
$C_{\text{sp}}$ & Top-$k$ sparsemax 	& 0.09 & 0.88 & 0.76 & 89.00 & 87.50  	    & &	0.38 & 0.80 & 0.59 & 68.25 & 80.25   \\
\midrule
$C_{\text{ent}}$ & Selec. 1.5-entmax 	& 0.13 & 0.80 & 0.60 & 86.50 & 84.00 		& & 0.21 & 0.84 & 0.67 & 75.25 & 87.00   \\
$C_{\text{sp}}$ & Selec. sparsemax 		& 0.10 & 0.89 & 0.77 & 87.75 & 86.75 		& & 0.35 & 0.83 & 0.66 & 72.25 & 85.00   \\
% $C_{\text{bern}}$ & Bernoulli 			& 0.42 & 0.66 & 0.30 & 70.75 & 70.75 		& & 0.24 & 0.85 & 0.69 & 74.50 & 86.75  \\
% $C_{\text{hk}}$ & HardKuma 				& 0.58 & 0.60 & 0.17 & 67.00 & 68.00 		& &	0.18 & 0.86 & 0.72 & 79.25 & 87.50 	\\
$C_{\text{bern}}$ & Bernoulli 			& 0.25 & 0.72 & 0.43 & 79.00 & 75.00 		& & 0.24 & 0.85 & 0.69 & 74.50 & 86.75  \\
$C_{\text{hk}}$ & HardKuma 				& 0.17 & 0.81 & 0.61 & 83.75 & 80.75 		& &	0.18 & 0.86 & 0.72 & 79.25 & 87.50 	\\
\midrule
$C$ & Joint $E$ and $L$ 				& 0.12 & 0.96 & 0.91 & 96.75 & 89.25 	    & &	0.65 & 0.71 & 0.44 & 58.00 & 70.00 	\\
- & Human highlights					& - & -   & -  & -  & -      		        & &	0.34 & 0.88 & 0.74 & 83.25 & 83.25 	\\
\midrule
% \multicolumn{2}{l}{\bf Average}         & \bf 0.20 & \bf 0.83 & \bf 0.65 & - & -    & & \bf 0.31 & \bf 0.82 & \bf 0.63 & - & - \\
\multicolumn{2}{l}{\bf Average}         & \bf 0.14 & \bf 0.85 & \bf 0.70 & - & -    & & \bf 0.31 & \bf 0.82 & \bf 0.63 & - & - \\
\bottomrule
\end{tabular}
\end{center}
\caption{Results for human evaluation. $\kappa$ is the Cohen's kappa coefficient, $p_o$ is the relative observed agreement, and $u$ represents the average of the portion of examples where annotators were unsure about their decisions.} 
\label{tab:table_agreement_human_eval}
\end{table}


% >>> np.mean(x1==x2)
% 0.845
% >>> cohen_kappa_score(x1,x2)
% 0.6854707792207793





\section{Examples of explanations}\label{sec:supp_explanations}

Tables \ref{table:word_overlap_imdb} and \ref{table:word_overlap_snli} show the average word overlap between explainers' messages ($m$) for IMDB and SNLI. Looking at the statistics we observed that, in general, top-$k$ attention-based classifiers produce similar explanations among themselves, and the erasure explainer produces messages similar to top-$k$ softmax. Major differences are observed for top-$k$ gradient and rationalizers, while selective attention produces, by definition, more words than top-$k$ attention (i.e. $m_{\text{top-k}} \subseteq m_{\text{selective}}$). It is worth noticing that although explainers with similar messages are expected to have a similar CSR (e.g. top-$k$ attention and erasure), including/excluding a single word in the explanation might impact the layperson decision, as we can see in the next examples. 
Tables \ref{table:examples_explanations_imdb_csrs} and \ref{table:examples_explanations_imdb_csrs2} show the output of erasure, gradient, attention, and joint explainers for IMDB, along with the prediction made by the classifier ($y_C$) and the layperson ($y_L$). In Tables \ref{table:examples_explanations_snli_csrs} and \ref{table:examples_explanations_snli_csrs2} we also include the human highlights explainer for SNLI. 
% In Table~\ref{table:examples_explanations_imdb_csrs} we show outputs for IMDB cases when the classifier and the layperson predicted a different label (decreasing CSR). Table~\ref{table:examples_explanations_snli_csrs} shows the same but for SNLI.

% \marcos{shuffle explanations in these tables? - except bernoulli and hardkuma? dont know}


\input{table_overlap_imdb.tex}
\input{table_overlap_snli.tex}

% \input{examples_expl_imdb_only.tex}
% \input{examples_expl_snli_only.tex}
\input{examples_expl_imdb_only_csrs.tex}
\input{examples_expl_snli_only_csrs.tex}



==> BlackBoxNLP 2020 - SCE/table_backup.tex <==
\begin{table*}[!htb]
\small

\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l cc c cc c cc c cc c cc}
\toprule
\multirow{2}{*}{\sc Explainer} & \multicolumn{2}{c}{\sc SST} & & \multicolumn{2}{c}{\sc IMDB} & & \multicolumn{2}{c}{\sc AgNews} & & \multicolumn{2}{c}{\sc Yelp} & & \multicolumn{2}{c}{\sc SNLI} \\


\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}  \cmidrule{14-15} 


	& CSR & ACC 	& & CSR & ACC 	& & CSR & ACC 	& & CSR & ACC 	& & CSR & ACC \\

\midrule 

BoW    	& -   & 82.54   	& & -   & 88.96  	& & -   & 95.62   	& & -   & 68.78   	& & -   & 69.81  \\
RNN softmax	        & -   & 86.16   	& & -   & 91.79  	& & -   & 96.28   	& & -   & 75.80   	& & -   & 78.34  \\
RNN 1.5-entmax		& -   & 86.11   	& & -   & 91.72  	& & -   & 96.30   	& & -   & 75.72   	& & -   & 79.20  \\
RNN sparsemax	 	& -   & 86.27   	& & -   & 91.52  	& & -   & 96.37   	& & -   & 75.72   	& & -   & 78.78  \\
Bernoulli		    & -   & 81.99   	& & -   & 87.65  	& & -   & 95.68   	& & -   & -   	& & -   & 85.69*  \\
HardKuma	    	& -   & 84.13   	& & -   & 90.52  	& & -   & 96.38   	& & -   & -   	& & -   & 85.49*  \\

\midrule 

%Top-$k$ Uniform	 		        & 68.31   & 68.86   	& & 66.77   & 66.47   	& & 92.44   & 91.26   	& & 58.27   & 53.03   	& & 75.44   & 68.24  \\
Random	        & 69.41   & 70.07   	& & 67.30   & 66.67   	& & 92.38   & 91.14   	& & 58.27   & 53.06   	& & 75.83   & 68.74  \\
% Top-$k$ max-out softmax	\andre{remove?}        & 75.34   & 75.23   	    & & 89.68   & 87.34   	    & & 96.33   & 94.79   	    & & 77.43   & 67.92   	& & 77.30   & 70.04  \\


Erasure   	    & 80.12   & 81.22   	    & & 92.17   & 88.72  	& & 97.31   & 95.41   	& & 78.72   & 68.90   	& & 77.88   & 70.04  \\
% Erasure 1.5-entmax \andre{remove?}  	& 84.51   & 83.03   	    & & 92.54   & 89.06  	& & 97.21   & 95.62   	& & 80.14   & 69.67   	& & 79.27   & 72.68  \\
% Erasure sparsemax \andre{remove?} 	& \bf 85.23   & 81.82   	& & 92.87   & 89.18  	& & 95.96   & 94.51   	& & 80.53   & 69.89   	& & 82.20   & 73.86  \\

%\midrule

Top-$k$ gradient       	& 79.35   & 79.24   	    & & 86.30   & 83.93  	    & & 96.49   & 94.86   	    & & 70.54   & 62.86   	& & 76.74   & 69.40  \\
Top-$k$ softmax	 	    & 84.18   & 82.43   	    & & 93.06   & 89.46   	    & & \bf 97.59   & 95.61   	& & 81.00   & 70.18   	& & 78.66   & 71.00  \\
Top-$k$ 1.5-entmax		& \bf 85.23   & \bf 83.31   & & 93.32   & 89.60   	    & & 97.29   & \bf 95.67   	& & 82.20   & 70.78   	& & 80.23   & 73.39  \\
Top-$k$ sparsemax	 	& \bf 85.23   & 81.93   	& & \bf 93.34   & 89.57   	& & 95.92   & 94.48   	    & & 82.50   & 70.99   	& & \bf 82.89   & \bf 74.76  \\

\midrule

Selec. 1.5-entmax			& 83.96   & 82.15   	    & & 92.55   & \bf 89.96   	& & 97.30   & 95.66   	& & 81.38   & 70.41   	        & & 77.25   & 71.44  \\
Selec. sparsemax	 		& \bf 85.23   & 81.93   	& & 93.24   & 89.66   	    & & 95.92   & 94.48   	& & \bf 83.55   & \bf 71.60   	& & 82.04   & 73.46  \\
Bernoulli	         		& 82.37   & 78.42   	    & & 90.27   & 86.45   	    & & 96.91   & 94.43   	& & -   & -   	                & & 72.46*   & 68.99*  \\
HardKuma	 		        & 85.17   & 80.40   	    & & 91.81   & 89.36   	    & & 97.11   & 95.45   	& & -   & -   	                & & 71.86*   & 68.70*  \\


\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results for text classification and SNLI datasets. CSR stands for the communication success rate, and ACC is the accuracy of the classifier/layperson. The top rows are the original classifiers, which access all words. %The erasure explainer is analogous to a wrapper method. 
The middle rows report performance for random, wrapper and filter explainers, for fixed $k$-word messages (the values of $k$ for the several datasets are \{5, 10, 10, 10, 4\}, respectively). The bottom rows correspond to embedded methods where $k$ is given automatically via sparsity. The average $k$ obtained by 1.5-entmax and sparsemax are: 
SST: \{4.65, 2.59\}; 
IMDB: \{28.23, 12.94\}; 
\textsc{AgNews} \{5.65, 4.14\};
\textsc{Yelp}: \{60.61, 23.86\}; 
SNLI: \{12.96, 8.27\}.
} \label{table:results_doc_classification}

\end{table*}

==> BlackBoxNLP 2020 - SCE/table_classifiers.tex <==
\begin{table}[t]
\small

\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{\hspace{2.5pt}}l@{\hspace{4.5pt}}p{.12\columnwidth}@{\hspace{4.5pt}}p{.12\columnwidth}@{\hspace{4.5pt}}p{.12\columnwidth}@{\hspace{4.5pt}}p{.12\columnwidth}@{\hspace{5pt}}p{.11\columnwidth}@{\hspace{0pt}}}

\toprule
{\sc Classifier} & 
{\sc SST} & {\sc IMDB} & {\sc AgN.} & {\sc Yelp} &{\sc SNLI} \\


\midrule 

{BoW ($L$)}   	&  {82.54}   	& {88.96}  	& {95.62}   	& {68.78}   	&  {69.81}  \\
{RNN, softmax ($C$)}	         & {86.16}   	 & {\bf 91.79}   & {96.28}   	 & {\bf 75.80}    & {78.34}  \\
{--,1.5-entmax ($C_{\text{ent}}$)}		& {86.11}   	 & {91.72}  	 & {96.30}   	 & {75.72}   	 & {79.20}  \\
{--, sparsemax	($C_{\text{sp}}$)} 	 & {\bf 86.27}    & {91.52}   & {96.37}   	 & {75.72}   	 & {78.78}  \\
% {Bernoulli ($C_{\text{bern}}$)}		     & {81.99}   	 & {87.65}  	 & {95.68}    & {75.06}   	 & {85.69*}  \\
% {Bernoulli ($C_{\text{bern}}$)}		     & {81.99}   	 & {87.65}  	 & {95.68}    & {70.12}   	 & {79.24}  \\
% {HardKuma ($C_{\text{hk}}$)}	    	 & {84.13}    & {90.52}   & {\bf 96.38}   	 & {74.36}   	& {\bf 85.49}  \\
{Bernoulli ($C_{\text{bern}}$)}		     & {81.99}    & {86.99}  	 & {95.68}    & {70.12}   	 & {79.24}  \\
{HardKuma ($C_{\text{hk}}$)}	    	 & {84.13}    & {91.06}   & {\bf 96.38}   	 & {74.36}   	& {\bf 85.49}  \\

\bottomrule
\end{tabular}
% }
\end{center}
\caption{Accuracies of the original classifiers on text classification and natural language inference.} 
\label{table:results_classifiers}

\end{table}

==> BlackBoxNLP 2020 - SCE/table_entropies_backup.tex <==
% THIS IS ON THE TEST SET

\begin{table}[!htb]
\small
\begin{center}
\begin{tabular}{ll ccc@{ }c ccc@{ }c}
\toprule
& & \multicolumn{3}{c}{\sc IMDB} & & \multicolumn{3}{c}{\sc SNLI} \\


\cmidrule{3-5} \cmidrule{7-9} 

\sc Clf. & \multirow{1}{*}{\sc Explainer} & $H$ & CSR & ACC$_L$  & & $H$ & CSR & ACC$_L$ \\
% Note: the CSR and ACC of these explainers are different from table 4 for IMDB because here we used k=5 (instead of k=10)
\midrule 
$C$         & Random                  & 9.62 	& 56.95 & 56.68 		& & 8.22 & 75.83 & 68.74     \\
$C$         & Erasure                 & 9.82 	& 91.73 & 88.04 		& & 9.69 & 77.88 & 70.04     \\
$C$         & Top-$k$ gradient        & 9.89 	& 81.61 & 79.46 		& & 9.35 & 76.74 & 69.40     \\
$C$         & Top-$k$ softmax         & 9.81 	& 91.96 & 88.17 		& & 9.76 & 78.66 & 71.00     \\
$C_{ent}$   & Top-$k$ 1.5-entmax      & 10.07   & 92.49 & 88.77 		& & 9.49 & 80.23 & 73.39     \\
$C_{sp}$    & Top-$k$ sparsemax       & 9.97 	& 92.82 & 88.88 		& & 8.80 & 82.89 & 74.76     \\

$C_{ent}$   & Select. 1.5-entmax      & 10.98 & 92.55 & 89.96 		& & 8.46 & 77.25 & 71.44     \\
$C_{sp}$    & Selec. sparsemax        & 10.69 & 93.24 & 89.66 		& & 8.37 & 82.04 & 73.46     \\
$C_{bern}$  & Bernoulli               & 9.75  & 90.27 & 86.45 		& & 8.25 & 76.81 & 69.65     \\
$C_{hk}$    & HardKuma                & 11.74 & 91.81 & 89.36 		& & 9.92 & 74.98 & 71.48     \\

$C_\star$   & Human highlights        & -     & -     & - 		    & & 9.27 & 81.32 & 81.32     \\
\midrule 
$C$         & Joint $E$ and $L$ ($\beta=0.0$)        & 6.39 & 93.54 & 90.14   	& & 9.80 & 81.66 & 73.44  \\
$C$         & Joint $E$ and $L$ ($\beta=0.2$)	     & 5.85 & 99.42 & 91.80   	& & 9.81 & 93.52 & 77.28  \\
$C$         & Joint $E$ and $L$ ($\beta=0.5$)	     & 5.77 & 99.82 & 91.74   	& & 9.45 & 95.81 & 77.54  \\
$C$         & Joint $E$ and $L$ ($\beta=1.0$)	     & 3.66 & 99.88 & 91.73   	& & 9.01 & 97.49 & 77.23  \\

\bottomrule
\end{tabular}
\end{center}
\caption{Entropy of the explanations for all explainers on IMDB and SNLI \andre{on the validation set?}. Entropy for human highlights was calculated based on non-neutral examples. $C_\star$ represents a classifier with a 100\% accuracy.
% Explanations for top-$k$ explainers were extracted using $k=5$.
% $S$ denotes the entropy of the explanations.
} 
\label{tab:results_joint_betas}
\end{table}

==> BlackBoxNLP 2020 - SCE/table_experiment.tex <==
\begin{table*}[!htb]
\small

\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ll c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r}
\toprule
& \sc Classifier & 
\multicolumn{2}{c}{\sc SST} & & \multicolumn{2}{c}{\sc IMDB} & & \multicolumn{2}{c}{\sc AgNews} & & \multicolumn{2}{c}{\sc Yelp} & & \multicolumn{2}{c}{\sc SNLI} \\


% \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}  \cmidrule{15-16} 

% \multicolumn{2}{l}{\sc Classifier}
% 	 & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} \\

\midrule 

$L$ & BoW    	& \multicolumn{2}{c}{82.54}   	& & \multicolumn{2}{c}{88.96}  	& & \multicolumn{2}{c}{95.62}   	& & \multicolumn{2}{c}{68.78}   	& & \multicolumn{2}{c}{69.81}  \\
$C$ & RNN softmax	        & \multicolumn{2}{c}{86.16}   	& & \multicolumn{2}{c}{91.79}  	& & \multicolumn{2}{c}{96.28}   	& & \multicolumn{2}{c}{75.80}   	& & \multicolumn{2}{c}{78.34}  \\
$C_{\text{ent}}$ & RNN 1.5-entmax		& \multicolumn{2}{c}{86.11}   	& & \multicolumn{2}{c}{91.72}  	& & \multicolumn{2}{c}{96.30}   	& & \multicolumn{2}{c}{75.72}   	& & \multicolumn{2}{c}{79.20}  \\
$C_{\text{sp}}$ & RNN sparsemax	 	& \multicolumn{2}{c}{86.27}   	& & \multicolumn{2}{c}{91.52}  	& & \multicolumn{2}{c}{96.37}   	& & \multicolumn{2}{c}{75.72}   	& & \multicolumn{2}{c}{78.78}  \\
$C_{\text{bern}}$ & Bernoulli		    & \multicolumn{2}{c}{81.99}   	& & \multicolumn{2}{c}{87.65}  	& & \multicolumn{2}{c}{95.68}   	& & \multicolumn{2}{c}{-}   	& & \multicolumn{2}{c}{85.69*}  \\
$C_{\text{hk}}$ & HardKuma	    	& \multicolumn{2}{c}{84.13}   	& & \multicolumn{2}{c}{90.52}  	& & \multicolumn{2}{c}{96.38}   	& & \multicolumn{2}{c}{-}   	& & \multicolumn{2}{c}{85.49*}  \\

\bottomrule
\toprule

\multirow{1}{*}{\sc Class.} & 
\multirow{1}{*}{\sc Explainer} & CSR & ACC & $|\mathcal{M}|$ & CSR & ACC & $|\mathcal{M}|$ & CSR & ACC & $|\mathcal{M}|$ & CSR & CSR & $|\mathcal{M}|$ & CSR & ACC & $|\mathcal{M}|$ \\

\midrule 

%Top-$k$ Uniform	 		        & 68.31   & 68.86   	& & 66.77   & 66.47   	& & 92.44   & 91.26   	& & 58.27   & 53.03   	& & 75.44   & 68.24  \\
$C$ & Random	        & 69.4   & 70.1   	& 5 & 67.3   & 66.7   	& 10 & 92.4   & 91.1   	& 10 & 58.3   & 53.1   	& 10 & 75.8   & 68.7 & 4 \\
% Top-$k$ max-out softmax	\andre{remove?}        & 75.34   & 75.23   	    & & 89.68   & 87.34   	    & & 96.33   & 94.79   	    & & 77.43   & 67.92   	& & 77.30   & 70.04  \\


$C$ & Erasure   	    & 80.1   & 81.2   	    & 5 & 92.2   & 88.7  	& 10 & 97.3   & 95.4   	& 10 & 78.7   & 68.9   	& 10 & 77.9   & 70.0 & 4 \\
% Erasure 1.5-entmax \andre{remove?}  	& 84.51   & 83.03   	    & & 92.54   & 89.06  	& & 97.21   & 95.62   	& & 80.14   & 69.67   	& & 79.27   & 72.68  \\
% Erasure sparsemax \andre{remove?} 	& \bf 85.23   & 81.82   	& & 92.87   & 89.18  	& & 95.96   & 94.51   	& & 80.53   & 69.89   	& & 82.20   & 73.86  \\

%\midrule

$C$ & Top-$k$ gradient       	& 79.4   & 79.2   	    & 5 & 86.3   & 83.9  	    & 10 & 96.5   & 94.9   	    & 10 & 70.5   & 62.9   	& 10 & 76.7   & 69.4 & 4  \\
$C$ & Top-$k$ softmax	 	    & 84.2   & 82.4   	    & 5 & 93.1   & 89.5   	    & 10 & \bf 97.6   & 95.6   	& 10 & 81.0   & 70.2   	& 10 & 78.7   & 71.0 & 4 \\
$C_{\text{ent}}$ & Top-$k$ 1.5-entmax		& \bf 85.2   & \bf 83.3   & 5 & 93.3   & 89.6   	    & 10 & 97.3   & \bf 95.7   	& 10 & 82.2   & 70.8   	& 10 & 80.2   & 73.4 & 4 \\
$C_{\text{sp}}$ & Top-$k$ sparsemax	 	& \bf 85.2   & 81.9   	& 5 & \bf 93.3   & 89.6   	& 10 & 95.9   & 94.5   	    & 10 & 82.5   & 71.0   	& 10 & \bf 82.9   & \bf 74.8 & 4 \\

\midrule

$C_{\text{ent}}$ & Selec. 1.5-entmax			& 84.0   & 82.2   	    & 4.7 & 92.6   & \bf 90.0   	& 28.2 & 97.3   & 95.7   	& 5.7 & 81.4   & 70.4   	        & 60.6 & 77.3   & 71.4 & 13.0 \\
$C_{\text{sp}}$ & Selec. sparsemax	 		& \bf 85.2   & 81.9   	& 2.6 & 93.2   & 89.7   	    & 12.9 & 95.9   & 94.5   	& 4.1 & \bf 83.6   & \bf 71.6   	& 23.9 & 82.0   & 73.5  & 8.3 \\
$C_{\text{bern}}$ & Bernoulli	         		& 82.4   & 78.4   	    & & 90.3   & 86.5   	    & & 96.9   & 94.4   	& & -   & -   	                & & 72.5*   & 69.0*  \\
$C_{\text{hk}}$ & HardKuma	 		        & 85.2   & 80.4   	    & & 91.8   & 89.4   	    & & 97.1   & 95.5   	& & -   & -   	                & & 71.9*   & 68.7*  \\


\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results for text classification and SNLI datasets. For each explainer, we indicate the corresponding classifier from Table~\ref{table:results_classifiers}; the layperson is a BoW model for all cases. CSR stands for the communication success rate, and ACC is the accuracy of the classifier/layperson. %The erasure explainer is analogous to a wrapper method. 
The top rows report performance for random, wrapper and filter explainers, for fixed $k$-word messages (the values of $k$ for the several datasets are \{5, 10, 10, 10, 4\}, respectively). The bottom rows correspond to embedded methods where $k$ is given automatically via sparsity. The average $k$ obtained by 1.5-entmax and sparsemax are: 
SST: \{4.65, 2.59\}; 
IMDB: \{28.23, 12.94\}; 
\textsc{AgNews} \{5.65, 4.14\};
\textsc{Yelp}: \{60.61, 23.86\}; 
SNLI: \{12.96, 8.27\}.
} \label{table:results_doc_classification}

\end{table*}

==> BlackBoxNLP 2020 - SCE/table_explainers.tex <==
\begin{table*}[!htb]
\small

\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l@{  }l cc@{ }c cc@{ }c cc@{ }c cc@{ }c cc}
\toprule
& & 
\multicolumn{2}{c}{\sc SST} & & \multicolumn{2}{c}{\sc IMDB} & & \multicolumn{2}{c}{\sc AgNews} & & \multicolumn{2}{c}{\sc Yelp} & & \multicolumn{2}{c}{\sc SNLI} \\


\cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}  \cmidrule{15-16} 

\sc Clf.\,\, & 
\multirow{1}{*}{\sc Explainer} & CSR & ACC$_L$ && CSR & ACC$_L$ && CSR & ACC$_L$ && CSR & ACC$_L$ && CSR & ACC$_L$ \\

\midrule 

%Top-$k$ Uniform	 		        & 68.31   & 68.86   	& & 66.77   & 66.47   	& & 92.44   & 91.26   	& & 58.27   & 53.03   	& & 75.44   & 68.24  \\
$C$ & Random	        & 69.41   & 70.07   	& & 67.30   & 66.67   	& & 92.38   & 91.14   	& & 58.27   & 53.06   	& & 75.83   & 68.74  \\
% Top-$k$ max-out softmax	\andre{remove?}        & 75.34   & 75.23   	    & & 89.68   & 87.34   	    & & 96.33   & 94.79   	    & & 77.43   & 67.92   	& & 77.30   & 70.04  \\


$C$ & Erasure   	    & 80.12   & 81.22   	    & & 92.17   & 88.72  	& & 97.31   & 95.41   	& & 78.72   & 68.90   	& & 77.88   & 70.04  \\
% Erasure 1.5-entmax \andre{remove?}  	& 84.51   & 83.03   	    & & 92.54   & 89.06  	& & 97.21   & 95.62   	& & 80.14   & 69.67   	& & 79.27   & 72.68  \\
% Erasure sparsemax \andre{remove?} 	& \bf 85.23   & 81.82   	& & 92.87   & 89.18  	& & 95.96   & 94.51   	& & 80.53   & 69.89   	& & 82.20   & 73.86  \\

%\midrule

$C$ & Top-$k$ gradient       	& 79.35   & 79.24   	    & & 86.30   & 83.93  	    & & 96.49   & 94.86   	    & & 70.54   & 62.86   	& & 76.74   & 69.40  \\
$C$ & Top-$k$ softmax	 	    & 84.18   & 82.43   	    & & 93.06   & 89.46   	    & & \bf 97.59   & 95.61   	& & 81.00   & 70.18   	& & 78.66   & 71.00  \\
$C_{\text{ent}}$ & Top-$k$ 1.5-entmax		& \bf 85.23   & \bf 83.31   & & 93.32   & 89.60   	    & & 97.29   & \bf 95.67   	& & 82.20   & 70.78   	& & 80.23   & 73.39  \\
$C_{\text{sp}}$ & Top-$k$ sparsemax	 	& \bf 85.23   & 81.93   	& & 93.34   & 89.57   	& & 95.92   & 94.48   	    & & 82.50   & 70.99   	& & \bf 82.89   & \bf 74.76  \\

\midrule

$C_{\text{ent}}$ & Selec. 1.5-entmax		& 83.96   & 82.15   	    & & 92.55   & 89.96   	& & 97.30   & 95.66   	& & 81.38   & 70.41   	        & & 77.25   & 71.44  \\
$C_{\text{sp}}$ & Selec. sparsemax	 		& \bf 85.23   & 81.93   	& & 93.24   & 89.66   	    & & 95.92   & 94.48   	& & 83.55   & 71.60   	        & & 82.04   & 73.46  \\
% $C_{\text{bern}}$ & Bernoulli	         	& 82.37   & 78.42   	    & & 90.27   & 86.45   	    & & 96.91   & 94.43   	& & 81.21   & 69.30   	        & & 72.46*   & 68.99*  \\

% $C_{\text{bern}}$  & Bernoulli	         	& 82.37   & 78.42   	    & & 90.27   & 86.45   	    & & 96.91   & 94.43   	& & 84.93   & 66.89   	        & & 76.81   & 69.65  \\
% $C_{\text{hk}}$ & HardKuma	 		        & 85.17   & 80.40   	    & & 91.81   & 89.36   	    & & 97.11   & 95.45   	& & \bf 87.39   & \bf 71.64   	& & 74.98   & 71.48  \\

$C_{\text{bern}}$  & Bernoulli	         	& 82.37   & 78.42   	    & & 91.66   & 86.13   	    & & 96.91   & 94.43   	& & 84.93   & 66.89   	        & & 76.81   & 69.65  \\
$C_{\text{hk}}$ & HardKuma	 		        & 85.17   & 80.40   	    & & \bf 94.72   & \bf 90.16   	    & & 97.11   & 95.45   	& & \bf 87.39   & \bf 71.64   	& & 74.98   & 71.48  \\

% lambda0 is for bernoullis and selection for hardkumas
% SST: bernoulli_sparsity01     -> lambda0 = 0.01   and selection = 0.3
% IMDB: bernoulli_sparsity0003  -> lambda0 = 0.0003 and selection = 0.3
% AGNEWS: bernoulli_sparsity01  -> lambda0 = 0.01   and selection = 0.3
% YELP: bernoulli_sparsity01/   -> lambda0 = 0.01   and selection = 0.3
% SNLI: bernoulli_sparsity0003_fix_new_indep_qk/    -> lambda 0 = 0.0003 and selection = 0.1
% Hardkuma: 

% SNLI: bernoulli_sparsity001_fix_new_indep_qk/
% k: 14.72
% acc c: 80.00
% csr: 71.08
% acc l: 62.87

% SNLI: bernoulli_sparsity0003_fix_new_indep_qk/   (running again - acc l seems very low)
% k: 15.04
% acc c: 79.24
% csr: 75.37 | 76.81
% acc l: 68.62 | 69.65




\bottomrule
\end{tabular}
% }
\end{center}
\caption{CSR and layperson accuracy (ACC$_L$) for several explainers. For each explainer, we indicate the corresponding classifier from Table~\ref{table:results_classifiers}; in all cases the layperson is a BoW model. 
Only explainers of the same classifier can be compared in terms of CSR.
Top rows report performance for random, wrapper and filter explainers, for fixed $k$-word messages (the values of $k$ for the several datasets are \{5, 10, 10, 10, 4\}, respectively). Bottom rows correspond to embedded methods where $k$ is given automatically via sparsity.
The average $k$ obtained by 1.5-entmax, sparsemax, Bernoulli and HardKuma are: 
SST: \{4.65, 2.59, 6.10, 4.82\}; 
% IMDB: \{28.23, 12.94, 61.46, 74.29\}; 
IMDB: \{28.23, 12.94, 39.40, 24.18\}; 
\textsc{AgNews} \{5.65, 4.14, 4.01, 9.68\};
\textsc{Yelp}: \{60.61, 23.86, 9.15, 33.18\}; 
SNLI: \{12.96, 8.27, 15.04, 6.40\}. 
} 
% \marcos{SNLI uses the decomposable attention classifier}
% \marcos{I see three options here: 1) change the classifier for all datasets to be a rnn with attention as we have before, and we test it with bernoulli and hardkuma attention. 2) we implement a generator-style model for SNLI based on bernoulli and hardkuma selection - this would be more faithful with the Lei et al model. 3) use a bernoulli attention version of the decomposable attention classifier (I'm working on this right now) - this would be more faithful with the Bastings et al model.}
\label{table:results_doc_classification}

\end{table*}

==> BlackBoxNLP 2020 - SCE/table_human.tex <==
\begin{table*}[t]
\small
\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ll ccccc c ccccc}
\toprule
\multirow{2}{*}{\sc Clf.} &
\multirow{2}{*}{\sc Explainer} & \multicolumn{5}{c}{IMDB} & & \multicolumn{5}{c}{SNLI} \\
\cmidrule{3-7}
\cmidrule{9-13}
        & & $k$ & CSR$_H$ & CSR$_L$ & ACC$_H$ & ACC$_L$         & & $k$ & CSR$_H$ & CSR$_L$ & ACC$_H$ & ACC$_L$ \\    
\midrule 

$C$ & Erasure 	                        & 5.0 & 89.25 & 94.00 & 86.25 & 90.00 		& & 4.0 & 72.50 & 73.50 & 83.50 & 70.00   \\
$C$ & Top-$k$ gradient 					& 5.0 & 73.50 & 84.50 & 73.00 & 80.50 	    & &	4.0 & 65.75 & 72.50 & 76.75 & 68.00    \\
$C$ & Top-$k$ softmax 					& 5.0 & 89.25 & 93.00 & 88.25 & 88.00 	    & &	4.0 & 72.00 & 76.50 & 82.75 & 71.50   \\
$C_{\text{ent}}$ & Top-$k$ 1.5-entmax 	& 5.0 & 89.25 & 92.50 & 85.75 & 86.50  	    & &	4.0 & 70.00 & 81.50 & 80.50 & 76.50   \\
$C_{\text{sp}}$ & Top-$k$ sparsemax 	& 5.0 & 89.00 & 89.50 & 87.50 & 88.00  	    & &	4.0 & 68.25 & 88.00 & 80.25 & 77.00   \\
\midrule
$C_{\text{ent}}$ & Selec. 1.5-entmax 	& 27.2 & 86.50 & 92.50 & 84.00 & 89.50 		& & 12.9 & 75.25 & 77.00 & 87.00 & 77.00   \\
$C_{\text{sp}}$ & Selec. sparsemax 		& 12.8 & 87.75 & 92.50 & 86.75 & 89.00 		& & 8.0  & 72.25 & 82.00 & 85.00 & 79.00   \\
% $C_{\text{bern}}$ & Bernoulli 			& 57.9 & 70.75 & 92.00 & 70.75 & 86.00 		& & 15.2 & 74.50 & 76.00 & 86.75 & 69.50  	\\
% $C_{\text{hk}}$ & HardKuma 				& 67.2 & 67.00 & 92.00 & 68.00 & 86.50 		& &	6.4  & 79.25 & 71.50 & \bf 87.50 & 68.50 	\\
$C_{\text{bern}}$ & Bernoulli 			& 39.4 & 79.00 & 93.50 & 75.00 & 87.00 		& & 15.2 & 74.50 & 76.00 & 86.75 & 69.50  	\\
$C_{\text{hk}}$ & HardKuma 				& 24.3 & 83.75 & 93.50 & 80.75 & 89.00 		& &	6.4  & 79.25 & 71.50 & \bf 87.50 & 68.50 	\\
\midrule
$C$ & Joint $E$ and $L$ 				& 2.7  & \bf 96.75 & \bf 98.50 & \bf 89.25 & \bf 91.50 	    & &	2.8 & 58.00 & \bf 93.50 & 70.00 & 78.50 	\\
- & Human highlights					& -  & -     & -     & -     & -                            & &	2.8 & \bf 83.25  & 83.50 & 83.25 & \bf 83.50 \\
% - & Human highlights					& -  & -     & -     & -     & -      	& &	3 & 69.00 & 76.00 & \bf 86.50 & 77.00 \\
% H CSR and L CSR nao faz muito sentido!
\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results of the human evaluation. Reported are average message length $k$, human layperson CSR$_H$/ACC$_H$, and machine layperson  CSR$_L$/ACC$_L$. 
% \andre{need to report message size of non-top-$k$ methods, and for human highlights we should have $CSR=ACC$}
Only explainers of the same classifier can be compared in terms of CSR.
} 
\label{table:results_human}
\end{table*}


==> BlackBoxNLP 2020 - SCE/table_human_backup.tex <==
\begin{table*}[t]
\small
\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l cccc c cccc}
\toprule
\multirow{2}{*}{\sc Explainer} & \multicolumn{4}{c}{IMDB} & & \multicolumn{4}{c}{SNLI} \\
\cmidrule{2-5}
\cmidrule{7-10}
        & $H$-CSR & $L$-CSR & $H$-ACC & $L$-ACC         & & $H$-CSR & $L$-CSR & $H$-ACC & $L$-ACC \\    
\midrule 

% 0.9915	0.7891

Top-$k$ gradient 	& 73.75 & 84.50 & 70.75 & 80.50 	            & &	66.00 & 76.00 & 78.50 & 75.00 \\
Top-$k$ softmax 	& 88.50 & 93.00 & 87.00 & 88.00 	            & &	70.50 & 75.00 & 81.00 & 74.00 \\
Top-$k$ 1.5-entmax 	& 87.50 & 92.50 & 85.00 & 86.50 	            & &	\bf 74.50 & 80.00 & 85.00 & 76.00 \\
Top-$k$ sparsemax 	& 90.00 & 89.50 & \bf 89.50 & 88.00 	        & &	73.00 & 86.00 & 81.50 & 76.00 \\
Joint $E$ and $L$ 	& \bf 93.25 & \bf 99.50 & 87.75 & \bf 92.50 	& &	72.00 & \bf 99.00 & 78.00 & \bf 80.00 \\
Human highlights	& -     & -     & -     & -      	            & &	69.00 & 76.00 & \bf 86.50 & 77.00 \\
% H CSR and L CSR nao faz muito sentido!
\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results for human evaluation. $H$-CSR/ACC stands for human annotator (layperson) performance, 
% in terms of success communication rate and accuracy on the real task, respectively. 
$L$-CSR/ACC stand for machine layperson performance.} \label{table:results_human}
\end{table*}


% 1-COLUMN VERSION [CSR ONLY]
% \begin{table}[t]
% \small
% \begin{center}
% \resizebox{1.0\columnwidth}{!}{%
% \begin{tabular}{l cc c cc}
% \toprule
% \multirow{2}{*}{\sc Explainer} & \multicolumn{2}{c}{IMDB} & & \multicolumn{2}{c}{SNLI} \\
% \cmidrule{2-3}
% \cmidrule{5-6}
%         & $H$-CSR & $L$-CSR         & & $H$-CSR & $L$-CSR \\    
% \midrule 

% % 0.9915	0.7891

% Top-$k$ gradient 	& 73.75 & 84.50 	        & &	66.00 & 76.00 \\
% Top-$k$ softmax 	& 88.50 & 93.00 	        & &	70.50 & 75.00 \\
% Top-$k$ 1.5-entmax 	& 87.50 & 92.50 	        & &	\bf 74.50 & 80.00 \\
% Top-$k$ sparsemax 	& 90.00 & 89.50 	        & &	73.00 & 86.00 \\
% Joint $E$ and $L$ 	& \bf 93.25 & \bf 99.50 	& &	72.00 & \bf 99.00 \\
% Human highlights	& -     & -      	        & &	69.00 & 76.00 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{Results for human evaluation. $H$-CSR represents the annotator performance.
% % in terms of success communication rate and accuracy on the real task, respectively. 
% $L$-CSR represents the layperson performance.} \label{table:results_human}
% \end{table}



==> BlackBoxNLP 2020 - SCE/table_overlap_imdb.tex <==
\begin{table}[!htb]
\scriptsize
\begin{center}

\begin{tabular}{@{}lllllllllll@{}}
\toprule

& Erasure 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\gradient\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\softmax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\1.5-entmax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\sparsemax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Selec.\\1.5-entmax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Selec.\\sparsemax\end{tabular} 
& Bernoulli 
& HardKuma 
& Joint $E$ and $L$ \\
\midrule 
Erasure             & \emph{1.00}  & 0.34  & 0.85  & 0.56  & 0.55  & 0.20  & 0.37  & 0.14  & 0.23  & 0.20 \\ 
Top-$k$ gradient    & 0.34	& \emph{1.00}	& 0.35	& 0.30	& 0.30	& 0.16	& 0.26	& 0.11	& 0.18	& 0.11 \\
Top-$k$ softmax     & 0.85	& 0.35	& \emph{1.00}	& 0.57	& 0.55	& 0.20	& 0.37	& 0.14	& 0.24	& 0.20 \\
Top-$k$ 1.5-entmax  & 0.56	& 0.30	& 0.57	& \emph{1.00}	& 0.61	& 0.21	& 0.39	& 0.12	& 0.24	& 0.19 \\
Top-$k$ sparsemax   & 0.55	& 0.30	& 0.55	& 0.61	& \emph{1.00}	& 0.20	& 0.43	& 0.13	& 0.24	& 0.20 \\
Selec. 1.5-entmax   & 0.20	& 0.16	& 0.20	& 0.21	& 0.20	& \emph{1.00}	& 0.45	& 0.24	& 0.44	& 0.08 \\
Selec. sparsemax    & 0.37	& 0.26	& 0.37	& 0.39	& 0.43	& 0.45	& \emph{1.00}	& 0.21	& 0.41	& 0.13 \\
Bernoulli           & 0.14	& 0.11	& 0.14	& 0.12	& 0.13	& 0.24	& 0.21	& \emph{1.00}	& 0.28	& 0.06 \\
HardKuma            & 0.23	& 0.18	& 0.24	& 0.24	& 0.24	& 0.44	& 0.41	& 0.28	& \emph{1.00}	& 0.08 \\
Joint $E$ and $L$   & 0.20	& 0.11	& 0.20	& 0.19	& 0.20	& 0.08	& 0.13	& 0.06	& 0.08	& \emph{1.00} \\


\bottomrule
\end{tabular}
\end{center}
\caption{Average word overlap (\%) between explainers for IMDB.} 
\label{table:word_overlap_imdb}
\end{table}

==> BlackBoxNLP 2020 - SCE/table_overlap_snli.tex <==
\begin{table}[!htb]
\scriptsize
\begin{center}

\begin{tabular}{@{}lllllllllll@{}}
\toprule

& Erasure 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\gradient\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\softmax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\1.5-entmax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Top-$k$\\sparsemax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Selec.\\1.5-entmax\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Selec.\\sparsemax\end{tabular} 
& Bernoulli 
& HardKuma 
& Joint $E$ and $L$ \\
\midrule 
Erasure             & \emph{1.00} & 0.38 & 0.77 & 0.55 & 0.41 & 0.35 & 0.37 & 0.32 & 0.49 & 0.38 \\
Top-$k$ gradient    & 0.38 & \emph{1.00} & 0.40 & 0.36 & 0.31 & 0.34 & 0.33 & 0.32 & 0.35 & 0.26 \\
Top-$k$ softmax     & 0.77 & 0.40 & \emph{1.00} & 0.56 & 0.41 & 0.36 & 0.37 & 0.32 & 0.49 & 0.38 \\
Top-$k$ 1.5-entmax  & 0.55 & 0.36 & 0.56 & \emph{1.00} & 0.46 & 0.36 & 0.42 & 0.32 & 0.46 & 0.34 \\
Top-$k$ sparsemax   & 0.41 & 0.31 & 0.41 & 0.46 & \emph{1.00} & 0.35 & 0.54 & 0.32 & 0.38 & 0.29 \\
Selec. 1.5-entmax   & 0.36 & 0.34 & 0.36 & 0.36 & 0.35 & \emph{1.00} & 0.64 & 0.88 & 0.48 & 0.26 \\
Selec. sparsemax    & 0.37 & 0.33 & 0.37 & 0.42 & 0.54 & 0.64 & \emph{1.00} & 0.60 & 0.45 & 0.26 \\
Bernoulli           & 0.32 & 0.32 & 0.32 & 0.32 & 0.32 & 0.88 & 0.60 & \emph{1.00} & 0.46 & 0.24 \\
HardKuma            & 0.49 & 0.35 & 0.49 & 0.46 & 0.38 & 0.48 & 0.45 & 0.46 & \emph{1.00} & 0.38 \\
Joint $E$ and $L$   & 0.38 & 0.26 & 0.38 & 0.34 & 0.29 & 0.26 & 0.26 & 0.24 & 0.38 & \emph{1.00} \\


\bottomrule
\end{tabular}
\end{center}
\caption{Average word overlap (\%) between explainers for SNLI.} 
\label{table:word_overlap_snli}
\end{table}

==> backup_tables.tex <==
\begin{table}[!htb]
\small
\begin{center}
\begin{tabular}{l cc c cc}
\toprule
\multirow{2}{*}{\sc Method} & \multicolumn{2}{c}{\sc SNLI} & & \multicolumn{2}{c}{\sc eSNLI} \\


\cmidrule{2-3} \cmidrule{5-6}


	& $C_{\mathrm{ACC}}$ & $L_{\mathrm{ACC}}$ 	& & $C_{\mathrm{ACC}}$ & $L_{\mathrm{ACC}}$  \\

\midrule 

Bag of words    	& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
RNN softmax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
RNN sparsemax	 	& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
RNN 1.5-entmax		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\

\midrule

Uniform	 		        & 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Shuffle	 		        & 86.20   & 86.20   	& & 86.20   & 86.20   	\\

\midrule 

Erasure softmax 		& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
Erasure sparsemax		& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
Erasure 1.5-entmax	    & 86.20   & 86.20   	& & 86.20   & 86.20  	\\

\midrule

Top-k gradient    		& 86.20   & 86.20   	& & 86.20   & 86.20  	\\
Zero-max-out softmax	& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Top-k softmax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Top-k sparsemax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Top-k 1.5-entmax		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\


\midrule

Full sparsemax	 		& 86.20   & 86.20   	& & 86.20   & 86.20   	\\
Full 1.5-entmax			& 86.20   & 86.20   	& & 86.20   & 86.20   	\\

\bottomrule
\end{tabular}
\end{center}
\caption{Results for SNLI and eSNLI.} \label{table:results_nli}
\end{table}




==> figs/experimental_comments.tex <==
\begin{itemize}
    \item Accuracy dos classifiers sao altas (muito proximo com os valores dos classifiers dos trabalhos relacionados - jain and wallace). 
    
    \item Falar do tamanho dos datsets nao influenciou muito
    
    \item Bag of words parece ser um strong baseline para todos os datasets. Especialmente para o AgNews
    
    \item Como esperado, usando shuffled or uniform random weights os resultados em termos de Lacc sao baixos. Exceto para o agnews, o qual usando random weights os resultados do layperson ainda sao consideravelmente altos (>90\%).
    
    \item Metodos baseados em erasure e encoded attention tem performances bem similares em termos de Lacc
    
    \item Gradient tem resultados mais baixos que erasure e attention
    
    \item Full attention (embedded) possui os melhores resultados em termos de Lacc
    
    \item Zerando a palavra com maior attention os resultados decaem comparando quando essa palavra estava inclusa, porem nao decaem tanto como quanto random, sugerindo que as palavras selecionadas via attention sao de fato relevantes. De fato, a acc desse explainer eh ate melhor que gradient explainer no IMDB e no YELP, os quais possuem sentencas muito grandes. Embora nao reportamos na tabela, resultados zerando os maiores attention scores computados via sparse attentions sao em geral um pouco melhores que usando softmax, entao a conclusao se mantem para alpha = 1.5 e 2.
    
    \item Usando attention ou erasure, os na maioria das vezes ficam melhores do que usando um bag of words completo, o que indica que a informacao relevante para a classificao esta sendo selecionada por esses explainers
    
    \item Com excecao do agnews, para os outros datasets da para perceber que sparse attentions geralmente refletem em uma maior accuracia de comunicacao. Para o agnews, descobrimos que se fizermos attention selecionando apenas as primeiras k palavras da sentenca, tanto a acc da comunicacao quanto a acc do layperson continuam muito altas (cerca de 93\%). Devido a isso, desconsideramos futuras analises para este corpus. 
    
    \item Olhando para a accuracia de comunicao podemos ver que metodos baseados em attention e erasure tambem possuem resultados melhores. 
    
    \item Novamente, olhando para os diferentes valores de alpha, percebemos que attentions mais esparsas tendem a ter uma acc de comunicacao ligeiramente maior (exceto no agnews).  
    
    \item Comparando os resultados entre encoded and embedded attention, podemos ver que em geral, a acc da comunicacao eh maior para encoded attention porem o layperson acc eh maior para embedded attention. Podemos ver tambem que para o SST e AgNews o resultado usando encoded e embedded sparsemax sao exatamente os mesmos. Isso acontece pois a distribuicao do sparsemax possui, na grande maioria das vezes, menos de $k$ nonzero probabilities, e portanto as mesmas palavras foram selecionadas pelos dois metodos. Mais adiante analisamos o impacto da esparsidade em mais detalhes.
    
    \item Em geral, esses experimentos nos mostram que, para os datasets analisados, usando palavras selecionadas via attention os resultados tanto em termos de Cacc e Lacc sao bastante apelativos, sugerindo que attention pode ser tratado como uma explicacao plausivel. Mais adiante discutimos se de fato podemos tratar as explanations desses metodos como faithfuls
\end{itemize}

==> table_backup.tex <==
\begin{table*}[!htb]
\small

\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l cc c cc c cc c cc c cc}
\toprule
\multirow{2}{*}{\sc Explainer} & \multicolumn{2}{c}{\sc SST} & & \multicolumn{2}{c}{\sc IMDB} & & \multicolumn{2}{c}{\sc AgNews} & & \multicolumn{2}{c}{\sc Yelp} & & \multicolumn{2}{c}{\sc SNLI} \\


\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}  \cmidrule{14-15} 


	& CSR & ACC 	& & CSR & ACC 	& & CSR & ACC 	& & CSR & ACC 	& & CSR & ACC \\

\midrule 

BoW    	& -   & 82.54   	& & -   & 88.96  	& & -   & 95.62   	& & -   & 68.78   	& & -   & 69.81  \\
RNN softmax	        & -   & 86.16   	& & -   & 91.79  	& & -   & 96.28   	& & -   & 75.80   	& & -   & 78.34  \\
RNN 1.5-entmax		& -   & 86.11   	& & -   & 91.72  	& & -   & 96.30   	& & -   & 75.72   	& & -   & 79.20  \\
RNN sparsemax	 	& -   & 86.27   	& & -   & 91.52  	& & -   & 96.37   	& & -   & 75.72   	& & -   & 78.78  \\
Bernoulli		    & -   & 81.99   	& & -   & 87.65  	& & -   & 95.68   	& & -   & -   	& & -   & 85.69*  \\
HardKuma	    	& -   & 84.13   	& & -   & 90.52  	& & -   & 96.38   	& & -   & -   	& & -   & 85.49*  \\

\midrule 

%Top-$k$ Uniform	 		        & 68.31   & 68.86   	& & 66.77   & 66.47   	& & 92.44   & 91.26   	& & 58.27   & 53.03   	& & 75.44   & 68.24  \\
Random	        & 69.41   & 70.07   	& & 67.30   & 66.67   	& & 92.38   & 91.14   	& & 58.27   & 53.06   	& & 75.83   & 68.74  \\
% Top-$k$ max-out softmax	\andre{remove?}        & 75.34   & 75.23   	    & & 89.68   & 87.34   	    & & 96.33   & 94.79   	    & & 77.43   & 67.92   	& & 77.30   & 70.04  \\


Erasure   	    & 80.12   & 81.22   	    & & 92.17   & 88.72  	& & 97.31   & 95.41   	& & 78.72   & 68.90   	& & 77.88   & 70.04  \\
% Erasure 1.5-entmax \andre{remove?}  	& 84.51   & 83.03   	    & & 92.54   & 89.06  	& & 97.21   & 95.62   	& & 80.14   & 69.67   	& & 79.27   & 72.68  \\
% Erasure sparsemax \andre{remove?} 	& \bf 85.23   & 81.82   	& & 92.87   & 89.18  	& & 95.96   & 94.51   	& & 80.53   & 69.89   	& & 82.20   & 73.86  \\

%\midrule

Top-$k$ gradient       	& 79.35   & 79.24   	    & & 86.30   & 83.93  	    & & 96.49   & 94.86   	    & & 70.54   & 62.86   	& & 76.74   & 69.40  \\
Top-$k$ softmax	 	    & 84.18   & 82.43   	    & & 93.06   & 89.46   	    & & \bf 97.59   & 95.61   	& & 81.00   & 70.18   	& & 78.66   & 71.00  \\
Top-$k$ 1.5-entmax		& \bf 85.23   & \bf 83.31   & & 93.32   & 89.60   	    & & 97.29   & \bf 95.67   	& & 82.20   & 70.78   	& & 80.23   & 73.39  \\
Top-$k$ sparsemax	 	& \bf 85.23   & 81.93   	& & \bf 93.34   & 89.57   	& & 95.92   & 94.48   	    & & 82.50   & 70.99   	& & \bf 82.89   & \bf 74.76  \\

\midrule

Selec. 1.5-entmax			& 83.96   & 82.15   	    & & 92.55   & \bf 89.96   	& & 97.30   & 95.66   	& & 81.38   & 70.41   	        & & 77.25   & 71.44  \\
Selec. sparsemax	 		& \bf 85.23   & 81.93   	& & 93.24   & 89.66   	    & & 95.92   & 94.48   	& & \bf 83.55   & \bf 71.60   	& & 82.04   & 73.46  \\
Bernoulli	         		& 82.37   & 78.42   	    & & 90.27   & 86.45   	    & & 96.91   & 94.43   	& & -   & -   	                & & 72.46*   & 68.99*  \\
HardKuma	 		        & 85.17   & 80.40   	    & & 91.81   & 89.36   	    & & 97.11   & 95.45   	& & -   & -   	                & & 71.86*   & 68.70*  \\


\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results for text classification and SNLI datasets. CSR stands for the communication success rate, and ACC is the accuracy of the classifier/layperson. The top rows are the original classifiers, which access all words. %The erasure explainer is analogous to a wrapper method. 
The middle rows report performance for random, wrapper and filter explainers, for fixed $k$-word messages (the values of $k$ for the several datasets are \{5, 10, 10, 10, 4\}, respectively). The bottom rows correspond to embedded methods where $k$ is given automatically via sparsity. The average $k$ obtained by 1.5-entmax and sparsemax are: 
SST: \{4.65, 2.59\}; 
IMDB: \{28.23, 12.94\}; 
\textsc{AgNews} \{5.65, 4.14\};
\textsc{Yelp}: \{60.61, 23.86\}; 
SNLI: \{12.96, 8.27\}.
} \label{table:results_doc_classification}

\end{table*}

==> table_entropies_backup.tex <==
% THIS IS ON THE TEST SET

\begin{table}[!htb]
\small
\begin{center}
\begin{tabular}{ll ccc@{ }c ccc@{ }c}
\toprule
& & \multicolumn{3}{c}{\sc IMDB} & & \multicolumn{3}{c}{\sc SNLI} \\


\cmidrule{3-5} \cmidrule{7-9} 

\sc Clf. & \multirow{1}{*}{\sc Explainer} & $H$ & CSR & ACC$_L$  & & $H$ & CSR & ACC$_L$ \\
% Note: the CSR and ACC of these explainers are different from table 4 for IMDB because here we used k=5 (instead of k=10)
\midrule 
$C$         & Random                  & 9.62 	& 56.95 & 56.68 		& & 8.22 & 75.83 & 68.74     \\
$C$         & Erasure                 & 9.82 	& 91.73 & 88.04 		& & 9.69 & 77.88 & 70.04     \\
$C$         & Top-$k$ gradient        & 9.89 	& 81.61 & 79.46 		& & 9.35 & 76.74 & 69.40     \\
$C$         & Top-$k$ softmax         & 9.81 	& 91.96 & 88.17 		& & 9.76 & 78.66 & 71.00     \\
$C_{ent}$   & Top-$k$ 1.5-entmax      & 10.07   & 92.49 & 88.77 		& & 9.49 & 80.23 & 73.39     \\
$C_{sp}$    & Top-$k$ sparsemax       & 9.97 	& 92.82 & 88.88 		& & 8.80 & 82.89 & 74.76     \\

$C_{ent}$   & Select. 1.5-entmax      & 10.98 & 92.55 & 89.96 		& & 8.46 & 77.25 & 71.44     \\
$C_{sp}$    & Selec. sparsemax        & 10.69 & 93.24 & 89.66 		& & 8.37 & 82.04 & 73.46     \\
$C_{bern}$  & Bernoulli               & 9.75  & 90.27 & 86.45 		& & 8.25 & 76.81 & 69.65     \\
$C_{hk}$    & HardKuma                & 11.74 & 91.81 & 89.36 		& & 9.92 & 74.98 & 71.48     \\

$C_\star$   & Human highlights        & -     & -     & - 		    & & 9.27 & 81.32 & 81.32     \\
\midrule 
$C$         & Joint $E$ and $L$ ($\beta=0.0$)        & 6.39 & 93.54 & 90.14   	& & 9.80 & 81.66 & 73.44  \\
$C$         & Joint $E$ and $L$ ($\beta=0.2$)	     & 5.85 & 99.42 & 91.80   	& & 9.81 & 93.52 & 77.28  \\
$C$         & Joint $E$ and $L$ ($\beta=0.5$)	     & 5.77 & 99.82 & 91.74   	& & 9.45 & 95.81 & 77.54  \\
$C$         & Joint $E$ and $L$ ($\beta=1.0$)	     & 3.66 & 99.88 & 91.73   	& & 9.01 & 97.49 & 77.23  \\

\bottomrule
\end{tabular}
\end{center}
\caption{Entropy of the explanations for all explainers on IMDB and SNLI \andre{on the validation set?}. Entropy for human highlights was calculated based on non-neutral examples. $C_\star$ represents a classifier with a 100\% accuracy.
% Explanations for top-$k$ explainers were extracted using $k=5$.
% $S$ denotes the entropy of the explanations.
} 
\label{tab:results_joint_betas}
\end{table}

==> table_experiment.tex <==
\begin{table*}[!htb]
\small

\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ll c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r c@{\hskip 5pt}c@{\hskip 5pt}r}
\toprule
& \sc Classifier & 
\multicolumn{2}{c}{\sc SST} & & \multicolumn{2}{c}{\sc IMDB} & & \multicolumn{2}{c}{\sc AgNews} & & \multicolumn{2}{c}{\sc Yelp} & & \multicolumn{2}{c}{\sc SNLI} \\


% \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}  \cmidrule{15-16} 

% \multicolumn{2}{l}{\sc Classifier}
% 	 & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} 	& & \multicolumn{2}{c}{ACC} \\

\midrule 

$L$ & BoW    	& \multicolumn{2}{c}{82.54}   	& & \multicolumn{2}{c}{88.96}  	& & \multicolumn{2}{c}{95.62}   	& & \multicolumn{2}{c}{68.78}   	& & \multicolumn{2}{c}{69.81}  \\
$C$ & RNN softmax	        & \multicolumn{2}{c}{86.16}   	& & \multicolumn{2}{c}{91.79}  	& & \multicolumn{2}{c}{96.28}   	& & \multicolumn{2}{c}{75.80}   	& & \multicolumn{2}{c}{78.34}  \\
$C_{\text{ent}}$ & RNN 1.5-entmax		& \multicolumn{2}{c}{86.11}   	& & \multicolumn{2}{c}{91.72}  	& & \multicolumn{2}{c}{96.30}   	& & \multicolumn{2}{c}{75.72}   	& & \multicolumn{2}{c}{79.20}  \\
$C_{\text{sp}}$ & RNN sparsemax	 	& \multicolumn{2}{c}{86.27}   	& & \multicolumn{2}{c}{91.52}  	& & \multicolumn{2}{c}{96.37}   	& & \multicolumn{2}{c}{75.72}   	& & \multicolumn{2}{c}{78.78}  \\
$C_{\text{bern}}$ & Bernoulli		    & \multicolumn{2}{c}{81.99}   	& & \multicolumn{2}{c}{87.65}  	& & \multicolumn{2}{c}{95.68}   	& & \multicolumn{2}{c}{-}   	& & \multicolumn{2}{c}{85.69*}  \\
$C_{\text{hk}}$ & HardKuma	    	& \multicolumn{2}{c}{84.13}   	& & \multicolumn{2}{c}{90.52}  	& & \multicolumn{2}{c}{96.38}   	& & \multicolumn{2}{c}{-}   	& & \multicolumn{2}{c}{85.49*}  \\

\bottomrule
\toprule

\multirow{1}{*}{\sc Class.} & 
\multirow{1}{*}{\sc Explainer} & CSR & ACC & $|\mathcal{M}|$ & CSR & ACC & $|\mathcal{M}|$ & CSR & ACC & $|\mathcal{M}|$ & CSR & CSR & $|\mathcal{M}|$ & CSR & ACC & $|\mathcal{M}|$ \\

\midrule 

%Top-$k$ Uniform	 		        & 68.31   & 68.86   	& & 66.77   & 66.47   	& & 92.44   & 91.26   	& & 58.27   & 53.03   	& & 75.44   & 68.24  \\
$C$ & Random	        & 69.4   & 70.1   	& 5 & 67.3   & 66.7   	& 10 & 92.4   & 91.1   	& 10 & 58.3   & 53.1   	& 10 & 75.8   & 68.7 & 4 \\
% Top-$k$ max-out softmax	\andre{remove?}        & 75.34   & 75.23   	    & & 89.68   & 87.34   	    & & 96.33   & 94.79   	    & & 77.43   & 67.92   	& & 77.30   & 70.04  \\


$C$ & Erasure   	    & 80.1   & 81.2   	    & 5 & 92.2   & 88.7  	& 10 & 97.3   & 95.4   	& 10 & 78.7   & 68.9   	& 10 & 77.9   & 70.0 & 4 \\
% Erasure 1.5-entmax \andre{remove?}  	& 84.51   & 83.03   	    & & 92.54   & 89.06  	& & 97.21   & 95.62   	& & 80.14   & 69.67   	& & 79.27   & 72.68  \\
% Erasure sparsemax \andre{remove?} 	& \bf 85.23   & 81.82   	& & 92.87   & 89.18  	& & 95.96   & 94.51   	& & 80.53   & 69.89   	& & 82.20   & 73.86  \\

%\midrule

$C$ & Top-$k$ gradient       	& 79.4   & 79.2   	    & 5 & 86.3   & 83.9  	    & 10 & 96.5   & 94.9   	    & 10 & 70.5   & 62.9   	& 10 & 76.7   & 69.4 & 4  \\
$C$ & Top-$k$ softmax	 	    & 84.2   & 82.4   	    & 5 & 93.1   & 89.5   	    & 10 & \bf 97.6   & 95.6   	& 10 & 81.0   & 70.2   	& 10 & 78.7   & 71.0 & 4 \\
$C_{\text{ent}}$ & Top-$k$ 1.5-entmax		& \bf 85.2   & \bf 83.3   & 5 & 93.3   & 89.6   	    & 10 & 97.3   & \bf 95.7   	& 10 & 82.2   & 70.8   	& 10 & 80.2   & 73.4 & 4 \\
$C_{\text{sp}}$ & Top-$k$ sparsemax	 	& \bf 85.2   & 81.9   	& 5 & \bf 93.3   & 89.6   	& 10 & 95.9   & 94.5   	    & 10 & 82.5   & 71.0   	& 10 & \bf 82.9   & \bf 74.8 & 4 \\

\midrule

$C_{\text{ent}}$ & Selec. 1.5-entmax			& 84.0   & 82.2   	    & 4.7 & 92.6   & \bf 90.0   	& 28.2 & 97.3   & 95.7   	& 5.7 & 81.4   & 70.4   	        & 60.6 & 77.3   & 71.4 & 13.0 \\
$C_{\text{sp}}$ & Selec. sparsemax	 		& \bf 85.2   & 81.9   	& 2.6 & 93.2   & 89.7   	    & 12.9 & 95.9   & 94.5   	& 4.1 & \bf 83.6   & \bf 71.6   	& 23.9 & 82.0   & 73.5  & 8.3 \\
$C_{\text{bern}}$ & Bernoulli	         		& 82.4   & 78.4   	    & & 90.3   & 86.5   	    & & 96.9   & 94.4   	& & -   & -   	                & & 72.5*   & 69.0*  \\
$C_{\text{hk}}$ & HardKuma	 		        & 85.2   & 80.4   	    & & 91.8   & 89.4   	    & & 97.1   & 95.5   	& & -   & -   	                & & 71.9*   & 68.7*  \\


\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results for text classification and SNLI datasets. For each explainer, we indicate the corresponding classifier from Table~\ref{table:results_classifiers}; the layperson is a BoW model for all cases. CSR stands for the communication success rate, and ACC is the accuracy of the classifier/layperson. %The erasure explainer is analogous to a wrapper method. 
The top rows report performance for random, wrapper and filter explainers, for fixed $k$-word messages (the values of $k$ for the several datasets are \{5, 10, 10, 10, 4\}, respectively). The bottom rows correspond to embedded methods where $k$ is given automatically via sparsity. The average $k$ obtained by 1.5-entmax and sparsemax are: 
SST: \{4.65, 2.59\}; 
IMDB: \{28.23, 12.94\}; 
\textsc{AgNews} \{5.65, 4.14\};
\textsc{Yelp}: \{60.61, 23.86\}; 
SNLI: \{12.96, 8.27\}.
} \label{table:results_doc_classification}

\end{table*}

==> table_human_backup.tex <==
\begin{table*}[t]
\small
\begin{center}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l cccc c cccc}
\toprule
\multirow{2}{*}{\sc Explainer} & \multicolumn{4}{c}{IMDB} & & \multicolumn{4}{c}{SNLI} \\
\cmidrule{2-5}
\cmidrule{7-10}
        & $H$-CSR & $L$-CSR & $H$-ACC & $L$-ACC         & & $H$-CSR & $L$-CSR & $H$-ACC & $L$-ACC \\    
\midrule 

% 0.9915	0.7891

Top-$k$ gradient 	& 73.75 & 84.50 & 70.75 & 80.50 	            & &	66.00 & 76.00 & 78.50 & 75.00 \\
Top-$k$ softmax 	& 88.50 & 93.00 & 87.00 & 88.00 	            & &	70.50 & 75.00 & 81.00 & 74.00 \\
Top-$k$ 1.5-entmax 	& 87.50 & 92.50 & 85.00 & 86.50 	            & &	\bf 74.50 & 80.00 & 85.00 & 76.00 \\
Top-$k$ sparsemax 	& 90.00 & 89.50 & \bf 89.50 & 88.00 	        & &	73.00 & 86.00 & 81.50 & 76.00 \\
Joint $E$ and $L$ 	& \bf 93.25 & \bf 99.50 & 87.75 & \bf 92.50 	& &	72.00 & \bf 99.00 & 78.00 & \bf 80.00 \\
Human highlights	& -     & -     & -     & -      	            & &	69.00 & 76.00 & \bf 86.50 & 77.00 \\
% H CSR and L CSR nao faz muito sentido!
\bottomrule
\end{tabular}
% }
\end{center}
\caption{Results for human evaluation. $H$-CSR/ACC stands for human annotator (layperson) performance, 
% in terms of success communication rate and accuracy on the real task, respectively. 
$L$-CSR/ACC stand for machine layperson performance.} \label{table:results_human}
\end{table*}


% 1-COLUMN VERSION [CSR ONLY]
% \begin{table}[t]
% \small
% \begin{center}
% \resizebox{1.0\columnwidth}{!}{%
% \begin{tabular}{l cc c cc}
% \toprule
% \multirow{2}{*}{\sc Explainer} & \multicolumn{2}{c}{IMDB} & & \multicolumn{2}{c}{SNLI} \\
% \cmidrule{2-3}
% \cmidrule{5-6}
%         & $H$-CSR & $L$-CSR         & & $H$-CSR & $L$-CSR \\    
% \midrule 

% % 0.9915	0.7891

% Top-$k$ gradient 	& 73.75 & 84.50 	        & &	66.00 & 76.00 \\
% Top-$k$ softmax 	& 88.50 & 93.00 	        & &	70.50 & 75.00 \\
% Top-$k$ 1.5-entmax 	& 87.50 & 92.50 	        & &	\bf 74.50 & 80.00 \\
% Top-$k$ sparsemax 	& 90.00 & 89.50 	        & &	73.00 & 86.00 \\
% Joint $E$ and $L$ 	& \bf 93.25 & \bf 99.50 	& &	72.00 & \bf 99.00 \\
% Human highlights	& -     & -      	        & &	69.00 & 76.00 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{Results for human evaluation. $H$-CSR represents the annotator performance.
% % in terms of success communication rate and accuracy on the real task, respectively. 
% $L$-CSR represents the layperson performance.} \label{table:results_human}
% \end{table}


